Deep Coregionalization for the Emulation of Spatial-Temporal Fields

Data-driven surrogate models are widely used for applications such as design optimization and uncertainty quantification, where repeated evaluations of an expensive simulator are required. For most partial differential equation (PDE) simulators, the outputs of interest are often spatial or spatial-temporal fields, leading to very high-dimensional outputs. Despite the success of existing data-driven surrogates for high-dimensional outputs, most methods require a significant number of samples to cover the response surface in order to achieve a reasonable degree of accuracy. This demand makes the idea of surrogate models less attractive considering the high computational cost to generate the data. To address this issue, we exploit the multi-fidelity nature of a PDE simulator and introduce deep coregionalization, a Bayesian non-parametric autoregressive framework for efficient emulation of spatial-temporal fields. To effectively extract the output correlations in the context of multi-fidelity data, we develop a novel dimension reduction technique, residual principal component analysis. Our model can simultaneously capture the rich output correlations and the fidelity correlations and make high-fidelity predictions with only a few expensive, high-fidelity simulation samples. We show the advantages of our model in three canonical PDE models and a fluid dynamics problem. The results show that the proposed method cannot only approximate a simulator with significantly less cost (at bout 10%-25%) but also further improve model accuracy.

==> intro_v1.tex <==
\section{Introduction}
%Gaussian process used as surrogate model for spatial-temporal field from computational models\\
%surrogate model 
Applications such as uncertainty quantification, design optimization and
inverse parameter estimation demand repeated simulations of partial differential equations (PDEs) in an input parameter space~\citep{Bilionis,Keane}.
Due to the high computational cost of a simulation, a data-driven surrogate model, also known as an emulator, is often employed in the place of the simulator~\citep{Kennedy2000,Santner2003}.
%Due to its rich model capacity and 
These surrogate models are essentially statical regression models that approximate the input-output mapping of the simulator~\citep{Santner2003}.
%Common models includes notably polynomial response surface models, Gaussian processes (GPs), and artificial neural networks.
%
%the problem of high dimension simulatin
Simulations of PDEs generally produce large spatial or spatial-temporal field results (e.g., velocity, temperature, or electric fields). Due to the large size, learning the results directly posed a huge challenge of model capacity and computational cost\citep{higdon2008computer,xing2015reduced,xing2016manifold}.
In some cases, this issue is avoided by only considering some concluding scaler values as the output of the surrogate models~\citep{Kennedy2000,Santner2003}.
This approach, however, disposes the valuable data that provides information into the simulator and potentially requires more data for model training~\citep{zhe2019scalable}.
In other cases, the quantity of interest could be the entire spatial-temporal field and the challenge is then inevitable\citep{higdon2008computer,xing2016manifold}.
%In this case, it is a common practice to first vectorize the field values at selected points in a spatial-temporal grid and consequently model the vector outputs in high-dimensional spaces.
In this case, modeling such outputs entails leaning the correlation between each output dimension effectively and efficiently.

% especially for problems requiring a fine resolution of the spatial characteristics, e.g., multiple spatial scales or moving boundaries.
\subsection{Gaussian process for high dimension outputs}
%Due to the capacity for uncertainty quantification and the non-parametric nature, 
As a non-parametric method that can also quantify model uncertainty, 
Gaussian process (GP) is frequently used as the main data-driven surrogate model~\citep{santner2003design,Kennedy2006,Rougier2009,Tagade2013,Lee2013}.
Unfortunately, the GP doest not naturally extended to multiple outputs, especially those of very large dimension such as spatial-temporal fields.  
It might seem straightforward to simply treat the output indexes (indicating the field value at a particular location in the spatial-temporal domain for instance) as additional input parameters~\citep{kennedy2001bayesian}.
This approach is infeasible for high dimensional outputs since the computational complexity for a general GP is $\mathcal{O}(N^3d^3)$, where $N$ is the number of training sample and $d$ is the output dimensionality~\citep{McFarland2008}.
If we can assume a separable structure between the input covariance and the output covariance, the high computational issues could be circumvented efficiently.
Such a relaxation gives rise to the linear model of coregionalization (LMC)~\citep{matheron1982pour, goulard1992linear},  the classical framework for multi-output regression.
LMC linearly combines some bases with latent processes to predict the high dimensional output.
Many modern multi-output GP models can be considered special instances or variants of LMC~\citep{Konomi2014,Fricker2013,Rougier2008,zhe2019scalable}.
\citet{Conti2010} proposed a simplified LMC model, known as intrinsic coregionalization model (ICM)~\citep{Wackernagel}, which assumes a single latent process with a correlation matrix governing output correlations.
To relax the limitation of ICM, \citet{higdon2008computer} found a set of bases from Singular Value Decomposition(SVD) on the training outputs to encode the complicated spatial-temporal correlations for PDE simulation problems.
This approach is further extended by using nonlinear dimension reduction, such as Kernel PCA~\citep{xing2016manifold} and Isomap~\citep{xing2015reduced}.
Once the bases are identified and fixed, we only need to learn a small number of latent process using ordinary univariate GPs~\citep{Rasmussen06GP}. 
Hence, LMC can easily scale up to a large number of outputs.
Recent development of GP further introduces latent coordinate features to improve the flexibility of modeling complex output correlations~\citep{zhe2019scalable}. 

The main drawback of LMC is the separable assumption, which can be resolved by \textit{process convolution}~\citep{higdon2002space, boyle2005dependent,teh2005semiparametric, bonilla2008multi}.
The key idea is to derive high dimension outputs based on convolution between a smoothing kernel and a set of latent process.
%Another line of high dimensional GP is based on convolution method between a smoothing kernel and a set of latent functions~\citep{higdon2002space,boyle2005dependent,teh2005semiparametric, bonilla2008multi}.
Despite their elegance, these methods are normally computationally costly. 
They have $\Ocal(N^3d^3)$ time complexity and hence are inappropriate for our application where the dimension is extremely large (\eg 1 million) while the samples are limited.
%To mitigate this issue, several sparse approximations have been developed~\citep{alvarez2009sparse,alvarez2010efficient}. 

%Despite their success, all these methods rely on single-fidelity data. 
\subsection{Autoregressive model for multi-fidelity data}
Since most data-driven surrogate models assume very little or no prior knowledge of the original PDE model, they normally require a large number of samples that well cover the response surface, in order to achieve a reasonable degree of accuracy.
It is not surprising that the number of training samples could grow drastically for a highly non-linear response surface.
In these cases, considering the huge amount of required experiments for generating the training data, the idea of surrogate models becomes less attractive.
One way to relax the high demand of training data is to inject prior knowledge of the PDE models to the surrogate models such as physical informed neural networks~\citep{raissi2019physics}, conservation kernels~\citep{macedo2010learning}, and hybrid physics based data-driven surrogates~\citep{shah2017reduced}.
%
Another way is to take the advantage of the multi-fidelity nature of a PDE simulator~\citep{kennedy2000predicting}.
Specifically, when generating training data for the data-driven surrogate models, we can easily reduce the computational cost by using a low fidelity simulator (e.g., a simulator with a sparser mesh) at the price of getting less accurate samples.
The low-fidelity samples, despite being noisy and biased, normally show strong correlation with the high-fidelity samples~\citep{kennedy2000predicting,damianou2013deep,perdikaris2017nonlinear,cutajar2019deep}.
If we can harness this correlation, we can model the system with many affordable low-fidelity samples and transfer the knowledge to predict highly accurate results without full reliance on highly accurate high-fidelity data.

The seminal work  of \citep{kennedy2000predicting} proposes an autoregressive method that learns the function of each fidelity as a linear combination of the function from the previous fidelity and a new function in the current fidelity. 
To relax the linear assumption in order to model more complicate problems, \citet{perdikaris2017nonlinear} used GP regression to learn the output of each fidelity as a nonlinear function of the current input and the output of the previous fidelity.
To fully capture and propagate the uncertainty throughout all fidelities, \citet{cutajar2019deep} jointly learned this chain GP model in the deep GP framework~\citep{damianou2013deep}.
As far as we are aware, there is no existing multi-fidelity models that deal with high dimensional output, which is often encountered for surrogate modeling.

In this paper,
We generalize the general autoregressive model using LMC to derive a deep LMC for modeling multi-fidelity high-dimensional simulation data. 
This general framework can simultaneously model the correlations between high dimensional outputs and those between different fidelity.
Furthermore, for the particular applications of high-dimensional simulation outputs, we develop residual principal component analysis -- an efficient method to build the deep LMC. 
% generalize the  nonlinear autoregressive model using the LMC framework for simultaneously modeling the correlations between high dimensional outputs and those between different fidelity.
The following paper is organized as followed:
first, we formulate our problems and briefly introduce the univariate GP for surrogate modeling. 
We then discuss its extension to multi-fidelity data, the general framework of GP autoregressive model. 
Following a discussion on the incapacity for high dimensional data, we generalize the GP autoregressive model for high dimensional data using the LMC framework. 
After some discussion on training of deep LMC, we introduce a residual principal component analysis algorithm to extract the bases for our model. 
Finally, we demonstrate the superiority of our method compared with existing high dimensional GPs on three fundamental PDEs, the Poisson's equation, the heat equation and the Burger's equation and a fluid dynamic problem, the lid-driven cavity.  



==> intro_v2.tex <==
\section{Introduction}
%Importance of emulation --->\\
Applications such as uncertainty quantification, design optimization and
inverse parameter estimation demand repeated simulations of partial differential equations (PDEs) in an input parameter space~\citep{Bilionis,Keane}.
Due to the high computational cost of a simulation, a data-driven surrogate model, also known as an emulator, is often employed in the place of the simulator~\citep{Kennedy2000,Santner2003}.
%Due to its rich model capacity and 
These surrogate models are essentially statical regression models that approximate the input-output mapping of the simulator~\citep{Santner2003}.
%Common models includes notably polynomial response surface models, Gaussian processes (GPs), and artificial neural networks.
%
%the problem of high dimension simulatin
Simulations of PDEs generally produce large spatial or spatial-temporal field results (e.g., velocity, temperature, or electric fields). Due to the large size, learning the results directly posed a huge challenge of model capacity and computational cost\citep{higdon2008computer,xing2015reduced,xing2016manifold}.




In some cases, this issue is avoided by only considering some concluding scaler values as the output of the surrogate models~\citep{Kennedy2000,Santner2003}.
%
%Modeling each output dimension independently disposes the valuable inter-output correlations and can lead to inferior model accuracy~\citep{zhe2019scalable}.
%Thus, it is crucial to learn the correlations between each output dimension effectively and efficiently.
%GAP: requirement of large dataset --->\\
This approach, however, disposes the valuable data that provides information into the simulator and potentially requires more data for model training~\citep{zhe2019scalable}.
In other cases, the quantity of interest can be the entire spatial-temporal field and the challenge is then inevitable\citep{higdon2008computer,xing2016manifold}.
%In this case, it is a common practice to first vectorize the field values at selected points in a spatial-temporal grid and consequently model the vector outputs in high-dimensional spaces.
Meanwhile, in order to achieve a reasonable degree of accuracy, a data-driven surrogate model requires a large number of samples that well cover the response surface.
%Since most data-driven surrogate models assume very little or no prior knowledge of the original PDE model, they normally require a large number of samples that well cover the response surface, in order to achieve a reasonable degree of accuracy.
It is not surprising that, for a highly non-linear response surface, the required number of training samples can grow drastically, which is impractical to satisfy due to the prohibit cost to generate all the training data.

Existing method--->\\
%In these cases, considering the huge amount of required experiments for generating the training data, the idea of surrogate models becomes less attractive.
One way to relax the high demand of training data is to inject prior knowledge of the PDE models to the surrogate models such as physical informed neural networks~\citep{raissi2019physics}, conservation kernels~\citep{macedo2010learning}, and hybrid physics based data-driven surrogates~\citep{shah2017reduced}.
Despite their success, these approaches cannot generalize well to all PDE problems and the implementations are not easy (neural networks requires massive model tunning; hybrid physics methods require modifying original simulation codes).
%
Another way is to take the advantage of the multi-fidelity nature of a PDE simulator~\citep{kennedy2000predicting,damianou2013deep,perdikaris2017nonlinear,cutajar2019deep}.
More specifically, when generating training data for the data-driven surrogate models, we can easily reduce the computational cost by using a low-fidelity simulator (e.g., a simulator with a sparse discretization mesh) at the price of getting less accurate samples.
The low-fidelity samples, despite of being noisy and biased, normally show strong correlation with the high-fidelity samples.
%Such a cross-fidelity correlation can be harnessed to 
By harnessing this correlation, we can model the system with many affordable low-fidelity samples and transfer the knowledge to predict highly accurate results without full reliance on highly accurate high-fidelity data.
%Another way is to take the advantage of the multi-fidelity nature of a PDE simulator~\citep{kennedy2000predicting}.
%Specifically, when generating training data for the data-driven surrogate models, we can easily reduce the computational cost by using a low fidelity simulator (e.g., a simulator with a sparser mesh) at the price of getting less accurate samples.
The seminal work of \citep{kennedy2000predicting} proposes an autoregressive method that assumes the function of each fidelity to be a linear transform from the previous fidelity.
This method is further extended by replacing the linear transformation with a GP regression to model more complicate problems~\citet{perdikaris2017nonlinear}.
To fully capture and propagate the uncertainty throughout all fidelities, \citet{cutajar2019deep} jointly learned this chain GP model in the deep GP framework~\citep{damianou2013deep}.
% learns the function of each fidelity as a linear combination of the function from the previous fidelity 
%and a new function in the current fidelity. 
%To relax the linear assumption in order to model more complicate problems, \citet{perdikaris2017nonlinear} used GP regression to learn the output of each fidelity as a nonlinear function of the current input and the output of the previous fidelity.
Despite of their great success, the existing multi-fidelity models consider only scalar output problems; they cannot directly apply to high-dimensional field problem because the input for the consequent fidelity GP would have excessively dimension (\eg 1 million).
Besides, it is unclear how to model the rich correlation between the high-dimensional field outputs to further improve the emulations.

To address this issues, we propose deep coregionalization, an efficient data-driven Bayesian surrogate framework for very high-dimensional spatial-temporal output simulations without fully reliance on expensive high-fidelity simulations.
Our model can simultaneously captures the correlation in spatial-temporal field and the correlations between different fidelity observations;
By fusing these correlations, our model can make accurate predictions of high-fidelity simulations with only a few expensive, high-fidelity experiments. Our contributions are as follows,
\begin{itemize}
	\item we generalize the deep auto-regressive model for high-dimensional output problems by integrating the classic linear model of coregionalization. We proof that with a mild assumption of a feasible linear decomposition for the fields, we can effectively propagate a compact underlying outputs correlations though a deep model to capture the cross-fidelity correlations and produce high-fidelity predictions.
	\item 
	To efficiently capture the output correlations of different fidelities without introducing a over-complicated models with many model parameters, 
%	reducing redundancy information (\ie the similar correlations across different fidelity), 
	we propose residual principal component analysis (ResPca), a dimension reduction technique that can effectively capture the meaningful correlations of high-dimension fields, efficiently preserve a compact representation for multi-fidelity fields, and easily scale to high dimension outputs (\eg 1 million).
	\item
	We validate the proposed method on 3 fundamental PDEs (Poisson's equation, Burgers' equation, and Heat equation) and a fluid dynamic problem. The results show a significant improvement not only on reducing the simulation budget (for generating the support data) but also on improving the predictive accuracy for the high-fidelity results.
	
\end{itemize}
%2) 
%We generalize the deep auto-regressive model based on the classic LMC framework and propose deep coregionalization, a theoretical framework for  the emulation of high-dimensional spatial-temporal fields from computational models.
%Our framework generalize very well to high-dimensional (\ie 1 million) field outputs and can 
%Our framework enables learning the correlations across multi-fidelity simulation data and the correlation between the high-dimensional outputs. Consequently, our model can achieve very high-fidelity predictions with only a few expensive, high-fidelity experiments.
%Our framework takes advantages of multi-fidelity simulation data to further improve accuracy for predictions.

%3)
%To efficiently capture the output correlations of different fidelities while reducing redundancy information (\ie the similar correlations across different fidelity), we propose residual PCA, a dimension reduction method that can compactly capture the correlations across different fidelity and easily scale to high dimension outputs (\eg 1 million).

%4)
%We validate the proposed method on 3 fundamental PDEs and a fluid dynamic problem. The results show a significant improvement not only on reducing the simulation budget (for generating the support data) but also on improving the predictive accuracy for high-fidelity results.




%and facilitate emulations of hihg
%In this paper,
%We generalize the general autoregressive model using LMC to derive a deep LMC for modeling multi-fidelity high-dimensional simulation data. 

%This general framework can simultaneously model the correlations between high dimensional outputs and those between different fidelity.
%
%Furthermore, for the particular applications of high-dimensional simulation outputs, we develop residual principal component analysis -- an efficient method to build the deep LMC. 
% generalize the  nonlinear autoregressive model using the LMC framework for simultaneously modeling the correlations between high dimensional outputs and those between different fidelity.
The following paper is organized as follows:
first, we formulate our problems and briefly introduce the univariate GP for surrogate modeling. 
We then discuss its extension to multi-fidelity data, the general framework of GP autoregressive model. 
Following a discussion on the incapacity for high dimensional data, we generalize the GP autoregressive model for high dimensional data using the LMC framework. 
After some discussion on training of deep LMC, we introduce a residual principal component analysis algorithm to extract the bases for our model. 
Finally, we demonstrate the superiority of our method compared with existing high dimensional GPs on three fundamental PDEs, the Poisson's equation, the heat equation and the Burger's equation and a fluid dynamic problem, the lid-driven cavity.  

Existing approach: autoregression --->
Issues: that can not deal with high dimensional problem --->
Our solutions: 

To address this issues, we propose deep cogerionaliztion, a Bayesian nonparametric framework, 

\subsection{Contribution}
1) 
%High-dimensional efficient 
We propose an efficient data-driven Bayesian surrogate framework for very-high dimensional spatial-temporal output simulations without fully reliance on expensive high-fidelity simulations.
Our model can simultaneously captures the strong correlation in spatial-temporal field and correlations between different fidelity observations.
As a result, our model can make accurate predictions of high-fidelity simulations with only a few expensive, high-fidelity experiments.

2) 
We generalize the deep auto-regressive model based on the classic LMC framework and propose deep coregionalization, a theoretical framework for  the emulation of high-dimensional spatial-temporal fields from computational models.
%Our framework generalize very well to high-dimensional (\ie 1 million) field outputs and can 
Our framework enables learning the correlations across multi-fidelity simulation data and the correlation between the high-dimensional outputs. Consequently, our model can achieve very high-fidelity predictions with only a few expensive, high-fidelity experiments.
%Our framework takes advantages of multi-fidelity simulation data to further improve accuracy for predictions.

3)
To efficiently capture the output correlations of different fidelities while reducing redundancy information (\ie the similar correlations across different fidelity), we propose residual PCA, a dimension reduction method that can compactly capture the correlations across different fidelity and easily scale to high dimension outputs (\eg 1 million).

4)
We validate the proposed method on 3 fundamental PDEs and a fluid dynamic problem. The results show a significant improvement not only on reducing the simulation budget (for generating the support data) but also on improving the predictive accuracy for high-fidelity results.


==> intro_v3.tex <==
\section{Introduction}
%Importance of emulation --->\\
Applications such as uncertainty quantification, design optimization and
inverse parameter estimation demand repeated simulations of partial differential equations (PDEs) in an input parameter space~\citep{Bilionis,Keane}.
Due to the high computational cost of a simulation, a data-driven surrogate model, also known as an emulator, is often employed in the place of the simulator~\citep{Kennedy2000,Santner2003}.
%Due to its rich model capacity and 
These surrogate models are essentially statical regression models that approximate the input-output mapping of the simulator~\citep{Santner2003}.
%Common models includes notably polynomial response surface models, Gaussian processes (GPs), and artificial neural networks.
%
%the problem of high dimension simulatin
In order to achieve a reasonable degree of accuracy, a data-driven surrogate model requires a large number of samples to well cover the response surface.
% due to the lack of applicable knowledge to the system
%Since most data-driven surrogate models assume very little or no prior knowledge of the original PDE model, they normally require a large number of samples that well cover the response surface, in order to achieve a reasonable degree of accuracy.
It is not surprising that, for a highly non-linear response surface, the required number of training samples can grow drastically, which is impractical to satisfy due to the prohibit cost to generate all the required training data.

%In this case, it is a common practice to first vectorize the field values at selected points in a spatial-temporal grid and consequently model the vector outputs in high-dimensional spaces.
%Meanwhile, in order to achieve a reasonable degree of accuracy, a data-driven surrogate model requires a large number of samples that well cover the response surface.
%Since most data-driven surrogate models assume very little or no prior knowledge of the original PDE model, they normally require a large number of samples that well cover the response surface, in order to achieve a reasonable degree of accuracy.
%It is not surprising that, for a highly non-linear response surface, the required number of training samples can grow drastically, which is impractical to satisfy due to the prohibit cost to generate all the training data.

%Existing method--->\\
%In these cases, considering the huge amount of required experiments for generating the training data, the idea of surrogate models becomes less attractive.
One way to relax the high demand of training data is to inject prior knowledge of the PDE models to the surrogate models such as physical informed neural networks~\citep{raissi2019physics}, conservation kernels~\citep{macedo2010learning}, and hybrid physics based data-driven surrogates~\citep{shah2017reduced}.
Despite their success, these approaches cannot generalize well to most PDE problems and the implementations are not easy (neural networks requires massive model tunning; hybrid physics methods require modifying original simulation codes).
%
Another way is to take the advantage of the multi-fidelity nature of a PDE simulator~\citep{kennedy2000predicting,damianou2013deep,perdikaris2017nonlinear,cutajar2019deep}.
More specifically, when generating training data for the data-driven surrogate models, we can easily reduce the computational cost by using a low-fidelity simulator (e.g., a simulator with a sparse discretization mesh) at the price of getting less accurate samples.
The low-fidelity samples, despite of being noisy and biased, normally show strong correlation with the high-fidelity samples.
%Such a cross-fidelity correlation can be harnessed to 
By harnessing this correlation, we can model the system with many affordable low-fidelity samples and transfer the knowledge to predict highly accurate results without full reliance on highly accurate high-fidelity data.
%Another way is to take the advantage of the multi-fidelity nature of a PDE simulator~\citep{kennedy2000predicting}.
%Specifically, when generating training data for the data-driven surrogate models, we can easily reduce the computational cost by using a low fidelity simulator (e.g., a simulator with a sparser mesh) at the price of getting less accurate samples.
The seminal work of \citep{kennedy2000predicting} proposes an autoregressive method that assumes the function of each fidelity to be a linear transform from the previous fidelity.
This method is further extended by replacing the linear transformation with a GP regression to model more complicate problems~\citet{perdikaris2017nonlinear}.
To fully capture and propagate the uncertainty throughout all fidelities, \citet{cutajar2019deep} jointly learned this chain GP model in the deep GP framework~\citep{damianou2013deep}.
% learns the function of each fidelity as a linear combination of the function from the previous fidelity 
%and a new function in the current fidelity. 
%To relax the linear assumption in order to model more complicate problems, \citet{perdikaris2017nonlinear} used GP regression to learn the output of each fidelity as a nonlinear function of the current input and the output of the previous fidelity.

Despite of their great success, existing multi-fidelity data-driven surrogates apply to only simple problems where the output is a scalar value. 
In practice, simulations of PDEs generally produce large spatial or spatial-temporal field results (e.g., velocity, temperature, or electric fields); the quantity of interest is often the entire spatial-temporal field\citep{higdon2008computer,xing2015reduced,xing2016manifold}.
%
In this case, the existing multi-fidelity methods cannot directly apply to high-dimensional field problem because the input for the consequent fidelity GP would have excessively dimension (\eg 1 million).
Besides, it is unclear how to model the rich correlation between the high-dimensional field outputs to improve the model performance.
%
\cmt{
Due to the large size, learning the results directly posed a huge challenge of model capacity and computational cost\citep{higdon2008computer,xing2015reduced,xing2016manifold}.
In some cases, this issue is avoided by only considering some concluding scaler values as the output of the surrogate models~\citep{Kennedy2000,Santner2003}.
%GAP: requirement of large dataset --->\\
This approach, however, disposes the valuable data that provides information into the simulator and potentially requires more data for model training~\citep{zhe2019scalable}.
In other cases, the quantity of interest can be the entire spatial-temporal field and the challenge is then inevitable\citep{higdon2008computer,xing2016manifold}.
}
To address this issues, we propose deep coregionalization, an efficient data-driven Bayesian surrogate framework for very high-dimensional spatial-temporal output simulations without fully reliance on expensive high-fidelity simulations.
Our model can simultaneously captures the correlation in spatial-temporal field and the correlations between different fidelity observations;
By fusing these correlations, our model can make accurate predictions of high-fidelity simulations with only a few expensive, high-fidelity experiments. Our contributions are as follows,
\begin{itemize}
	\item We generalize the deep auto-regressive model for high-dimensional output problems by integrating the classic linear model of coregionalization (LMC). We proof that with a mild assumption of separable structures, we can effectively propagate the output correlations though a deep model to capture the cross-fidelity correlations and produce high-fidelity predictions.
	\item 
	To efficiently capture the output correlations of different fidelities without introducing a over-complicated model with many model parameters, 
%	reducing redundancy information (\ie the similar correlations across different fidelity), 
	we propose residual principal component analysis (ResPca), a dimension reduction technique that can effectively capture the meaningful correlations of high-dimension fields, efficiently preserve a compact representation for multi-fidelity fields, and easily scale to high-dimensional field outputs (\eg 1 million).
	\item
	We validate the proposed method on 3 fundamental PDEs (Poisson's equation, Burgers' equation, and Heat equation) and a fluid dynamic problem. The results show a significant improvement not only on reducing the simulation budget (for generating the support data) but also on improving the predictive accuracy for the high-fidelity results, compared with models using single fidelity data.
	
\end{itemize}
%2) 
%We generalize the deep auto-regressive model based on the classic LMC framework and propose deep coregionalization, a theoretical framework for  the emulation of high-dimensional spatial-temporal fields from computational models.
%Our framework generalize very well to high-dimensional (\ie 1 million) field outputs and can 
%Our framework enables learning the correlations across multi-fidelity simulation data and the correlation between the high-dimensional outputs. Consequently, our model can achieve very high-fidelity predictions with only a few expensive, high-fidelity experiments.
%Our framework takes advantages of multi-fidelity simulation data to further improve accuracy for predictions.

%3)
%To efficiently capture the output correlations of different fidelities while reducing redundancy information (\ie the similar correlations across different fidelity), we propose residual PCA, a dimension reduction method that can compactly capture the correlations across different fidelity and easily scale to high dimension outputs (\eg 1 million).

%4)
%We validate the proposed method on 3 fundamental PDEs and a fluid dynamic problem. The results show a significant improvement not only on reducing the simulation budget (for generating the support data) but also on improving the predictive accuracy for high-fidelity results.




%and facilitate emulations of hihg
%In this paper,
%We generalize the general autoregressive model using LMC to derive a deep LMC for modeling multi-fidelity high-dimensional simulation data. 

%This general framework can simultaneously model the correlations between high dimensional outputs and those between different fidelity.
%
%Furthermore, for the particular applications of high-dimensional simulation outputs, we develop residual principal component analysis -- an efficient method to build the deep LMC. 
% generalize the  nonlinear autoregressive model using the LMC framework for simultaneously modeling the correlations between high dimensional outputs and those between different fidelity.
The following paper is organized as follows:
First, we formulate our problems and briefly introduce the univariate GP for surrogate modeling. 
We then discuss the general framework of GP autoregressive model, a GP extension using multi-fidelity data to reduce the reliance on large, high-fidelity training data. 
% its extension to multi-fidelity data, 
Following a discussion on the output correlations the LMC, we develop our proposed deep coregionalization model.
% on the incapacity for high dimensional data, we generalize the GP autoregressive model for high dimensional data using the LMC framework. 
After some discussion on training of deep LMC, we introduce the ResPca algorithm to extract compact representations of multi-fidelity data for our model.
Finally, we demonstrate the superiority of our method compared with existing high-dimensional GPs on three fundamental PDEs, the Poisson's equation, the heat equation and the Burger's equation and a fluid dynamic problem, the lid-driven cavity.  

%Existing approach: autoregression --->
%Issues: that can not deal with high dimensional problem --->
%Our solutions: 


==> model_v1.tex <==
\section{Statement of the problem}\label{emulate}
Consider a parameterized nonlinear system of steady-state or transient PDEs of arbitrary order for dependent variables (scalar fields) $u(\x,\s ,t)$, where $\x\in \mathbb{R}^l$ is a vector that parameterizes the PDEs, $\s$ and $t$ denotes spatial and temporal index.
% To give a concrete example, the $u_i$, $i=1,\hdots,4$, could refer to velocity components (say $i=1,2,3$) and pressure ($i=4)$ in a fluid flow model. 
The PDEs are permitted to be fully nonlinear and parameterized in an arbitrary fashion (including the initial and boundary conditions).
It is assumed  that the PDE model is well-posed (solutions exist and are unique) for the range of values of $\x$ considered.

The quantities of interest is the function $u(\x,\s,t)$ in given range.
Direct approximation of this function is difficult due to the amount of samples we need to cover the response surface for such a high dimensional space~\citep{higdon2008computer}.
Instead, we can record values at specified (fixed) spatial locations, $\s_i$, $i=1,\dots,d_s$, and temporal locations, $t_i$, $i=1,\dots,d_t$.
For different inputs parameters $\x_i\in \mathbb{R}^l$, the  outputs of the simulator are represented as vectors: $\y^{(F)}_i = \y^{(F)}(\x_i) = (u(\x_i,\s_1,t_1),...,u(\x_i,\s_{d_s},t_{d_t}))^T \in \mathbb{R}^d$, where $d=d_s\times d_t$. 
Here, we use the superscript ${(F)}$ to denote that resulting vector is from an accurate fine simulation.
%As is suggested in \citep{higdon2008computer},
The value at a different spatial-temporal locations can be achieved easily through interpolation provided that the spatial-temporal fixed points are dense enough which can be done easily with ignorable extra computational effort~\citep{higdon2008computer}.

From the preceding discussion, the simulation is now considered a mapping from $\mathbb{R}^l$ to $\mathbb{R}^d$, where $d$ is extremely large.
The goal of a data-driven surrogate is to approximate the mapping given {\/\it training points\/} $\mathcal{D} = \{\X, \Y^{(F)}\}$, where $\X = [\x_1,\ldots,\x_N]^T$ and $\Y^{(F)} = [\y^{(F)}_1,\ldots,\y^{(F)}_N]^T$.
%where $\y^{(F)}_i$ denotes the finest fidelity data that are very close to the ground truth value and the corresponding inputs $\x_i$ are referred to as {\/\it design inputs\/}. 
Provided enough number of samples covering the response surface, we can approximate the mapping accurately.
In practice, getting accurate high fidelity data is computational expensive; it is impractical to get enough samples to cover the response surface of our interest.
It is, however, practically easy to compromise the accuracy by ruining a simulator, given input $\x_i$ in a lower fidelity setting to collect cheaper but less accurate observation $\y_i^{(F-1)}$ and even cheaper observation $\y_i^{(F-2)}$.
We denote the all fidelity data by $\{\X^{(f)}, \Y^{(f)}\}_{f=1}^F$, where $\Y^{(f)}$ is a $N_f\times d$ matrix for observations at fidelity setting $i$ with $\X^{(f)}$ being a $N_f\times l$ matrix for the corresponding inputs.
Following the common setting for multi-fidelity data~\citep{perdikaris2017nonlinear,cutajar2019deep}, we also require that the training input of fidelity $f$ is a subset the previous fidelity $f-1$, .i.e, $\X^{(f)} \subset \X^{(f-1)}$. For convenience, 
% It is obvious that for $f\geq2$, $\X^{(f)} \subset \X^{(1)}$.
we introduce the index notation $\e$ to select raws form a standard matrix such that $\X^{(f)} = \X_{\e_f,:}$, where $\e_f$ indicating the subset for fidelity data $f$.


%It is assumed for now that a single output $\mbox{\textbf{\textit{y}}}$ (derived from a single scalar field $u({\textbf{\textit{x}}};{\pmb{\xi}})$) is the target for emulation. 
%
%From the preceding discussion, the simulator can be considered as a mapping $\pmb{\eta}:{\cal X}\rightarrow {\cal M}$ (assumed to be injective), where ${\cal M}\subset \mathbb{R}^d$ is the permissible output space (response surface) and ${\cal X} \subset \mathbb{R}^l$ is the permissible input space. That is, $\pmb{\eta}(\pmb{\xi})= \mbox{\textbf{\textit{y}}}=(u(\textbf{\textit{x}}^{(1)};\pmb{\xi}),\dots,u(\textbf{\textit{x}}^{(d)};\pmb{\xi}))^T$ for an arbitrary input $\pmb{\xi}$. 

%To infer outputs of the simulator at new inputs, Conti and O'Hagan~\cite{Conti2010} took the approach of placing a $d$-dimensional GP prior over $\pmb{\eta}$, indexed by $\pmb{\xi}$.  Effectively, the same assumption was made by Higdon {\/\em et al.\/}~\cite{Higdon} but in that case the outputs were a linear combination of PCA basis vectors with coefficients  treated as independent univariate GPs indexed by $\pmb{\xi}$. In this paper, a similar approach is adopted but rather than using PCA coefficients  we place GP priors over coefficients of a reduced-dimensional approximation of  points in ${\cal M}$, obtained by manifold learning methods. We assume that  ${\cal M}$ is a smooth manifold in $\mathbb{R}^d$. The high dimension $d$ of the output space  and the inability of linear dimensionality reduction methods such as PCA to capture complex response surfaces  is the motivation for our approach. 

\section{Model Formulation}
%problem definiteion --- deep gp (with introduction of sgp) --- lmc model --- deep lmc model 

\subsection{Univariate Gaussian Process}
We first review GP regression to learn a univariate function given a fine fidelity dataset $\Dcal = \{\X, \Y\}$. Here we omit the superscript ${(F)}$ for clarity but the data is assumed collected from of a fine (high-fidelity) simulator.
The quantity of interest is a univariate, i.e., $d=1$. We use $y_i$ to distinct the univariate observations from a multivariate one $\y_i$.
%where each $\x_i$ is a $l$ dimensional input vector, and $y^{(F)}_i$ the observed scalar output, we aim to learn a function $f: \mathbb{R}^p \rightarrow \mathbb{R}$. 
GP regression assumes the finite set of function values on $\X = [\x_1, \ldots, \x_N]^\top$, namely $\y = [y_1, \ldots, y_N]^\top$, follow a multivariate Gaussian distribution, 
$p(\y | \X) = \N(\y | \m, \K + \tau^{-1} \I)$.
Here $\m = [m(\x_1), \ldots, m(\x_n)]^\top$ is the mean function that is usually set to $\0$ after centering $\Y$~\citep{kennedy2001bayesian,rasmussen2003gaussian}.
$\tau$ is the inverse noise variance, that accounts for model inadequacies and numerical error.
$\K$ is the covariance matrix with elements $[\K]_{i,j} = k(\x_i, \x_j)$, where $k(\x_i, \x_j)$ is a kernel function of the corresponding inputs.
Choosing the right kernel function for a specific application is nontrivial. 
When there is nor prior knowledge to guide the choice, the automatic relevance deterrence (ARD) kernel \citep{rasmussen2003gaussian}, reading as,
\begin{equation}
	k(\x_i, \x_j) = \theta_0 \exp\left(-(\x_i-\x_j) \diag(\theta_1,\ldots,\theta_l) (\x_i-\x_j)^T \right)
\end{equation}
is normally implemented. The ARD kernel has $l+1$ hyperpameters that determine the impact of each input parameters and thus the name ARD.
%Each element of $\K$ is defined as a kernel function of the corresponding inputs: $[\K]_{i,j} = k(\x_i, \x_j)$.%, \eg ARD squared exponential kernel, $\mathrm{cov}\big(f(\x_i), f(\x_j)\big) = k(\x_i, \x_j) = \sigma_0^2 \exp\left(-\frac{1}{2} (\x_i-\x_j)^\top \diag(\Beta) (\x_i -\x_j)\right)$,
%where $\Beta = [1/\sigma_1^2, ..., 1/\sigma_p^2]$. 
%The model prior reads as $p(\y|\f) = \N(\y|\f, \tau^{-1}\I)$ where $\tau$ is the inverse noise variance, that accounts for model inadequacies and numerical error.
%To account for model inadequacies and numerical error, which is assumed Gaussian distributed, in the simulation model, the prior for the model reads as, $p(\y|\f) = \N(\y|\f, \tau^{-1}\I)$ where $\tau$ is the inverse noise variance. 
%The observed outputs  $\y = [y_1, \ldots, y_N]^\top$ are assumed to be corrupted, \eg by some Gaussian random noises, 
%We can marginalize out $\y$ to obtain the marginal likelihood of $\y$, $p(\y|\X) = \N\big(\y|\0, \K + \tau^{-1}\I\big)$.
Given a new input $\x_*$, we can derive its posterior using a conditional Gaussian distribution,
\begin{equation}
\label{eq:sgp}
\begin{aligned}
 p\big(y_*|\x_*, \X,\y\big) &= \N\left(y_* | \mu(\x_*), v(\x_*)\right) \\
 \mu(\x_*) &= \k_{*}^\top (\K + \tau^{-1} \I)^{-1}\y \\
 v(\x_*) &= k(\x_*, \x_*) - \k_{*}^\top(\K + \tau^{-1}\I)^{-1}\k_{*},
\end{aligned}
\end{equation}
where, $\k_{*} = [k(\x_*, \x_1), \ldots, k(\x_*, \x_N)]^\top$ is the covariance between $\x_*$ and $\X$. 
The inference of the GP regression is to estimate the covariance (or kernel) parameters (\eg $\{\theta_0, \ldots, \theta_l\}$ in the ARD  kernel) and the inverse noise variance $\tau$ that best explain the observed data $\Dcal$.
We can optimize these hyperparameters by maximizing  the  marginal likelihood likelihood,
\begin{equation}
\label{eq:sgp likelihood}
	\Lcal = \frac{1}{2} \ln|\K| - \frac{1}{2}\Y^T \K^{-1} \Y - \frac{N}{2} \ln(2\pi).
\end{equation}
The main computational cost is the inversion of $\K$, which takes $\Ocal(N^3)$ and $\Ocal(N^2)$ time and space complexity, respectively.

\subsection{Deep Gaussian Process}
Now, let us consider the multi-fidelity univariate data.
i.e., we have data $\{\X^{(f)},\Y^{(f)}\}_{f=1}^F$, where $\Y^{(f)} = [y^{(f)}_1,\ldots,y^{(f)}_{N_f}]^T $ is a collection of samples at fidelity $f$.
%First, let consider the traditional GP for multi-fidelity data where the quantity of interest is a univariate, i.e., $d=1$ for our problem. We use $y$ to distinct the univariate observations from a multivariate one $\y$.
The general formulation of autoregressive GP for multi-fidelity is,
% data put forward by \citep{perdikaris2017nonlinear} is
\begin{equation}
y^{(f)}(\x) = g^{(f)}\left(y^{(f-1)}(\x)\right) + \delta^{(f)}(\x),
\end{equation}
where $g^{(f)}(y^{(f-1)}(\x))$ is an arbitrary function that maps the low fidelity result to the high fidelity one and $\delta^{(f)}(\x)$ captures the noise.
If we assume a simple linear form of $g^{(f)}(\y^{(f-1)}(\x))$, i.e.,  $g^{(f)}(\y^{(f-1)}(\x)) = c \cdot \y^{(f-1)}(\x)$, we recover the classic autoregressive model of \citep{kennedy2000predicting}.
This method is further improved by \citet{le2013multi} using a deterministic parametric form of $g^{(f)}$ and an efficient numerical scheme to reduce the computational cost. 
Despite being successful to deal with many real problems, this parametric approach requires expert knowledge for the model selection as well as a large dataset for model training. This approach is not always feasible in the area of complex system simulation~\citep{perdikaris2017nonlinear}.
To resolve this issue, a Bayesian non-parametric treatment can be implemented by placing a GP prior over the function $g^{(f)}$.
This is also known as the \textit{deep GP}~\citep{damianou2013deep}.
Despite being capable of modeling complex problem, deep GPs are infamous for their intractability which results in computationally expensive variational approximation for model training.
Motivated by the work of \citep{le2013multi}, \citet{perdikaris2017nonlinear}, put forward an GP based nonlinear autoregressive scheme with an additive structure,
\begin{equation} \label{eq:deep gp}
y^{(f)}(\x) = g^{(f)}\left(\x, y_*^{(f-1)}(\x)\right),
\end{equation}
where the noise term is absorbed into $g^{(f)}(\x)$ and $y_*^{(f-1)}(\x) $ is the GP posterior of the previous level. 
%which is effective for the multi-fidelity problem.
To better reflect the autoregressive nature, the covariance function decomposes as,
\begin{equation}
\label{eq:deep sgp}
\begin{aligned}
&k^{(f)}\left(\x, \x', y_*^{(f-1)}(\x), y_*^{(f-1)}(\x)\right)\\ &=  k_x^{(f)}(\x, \x'; \btheta_{fx} ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x), y_*^{(f-1)}(\x'); \btheta_{fy} ) +k_{\delta}^{(f)}(\x, \x'; \btheta_{f\delta}),
\end{aligned}
\end{equation}
where $k_x^{(f)}$, $k_y^{(f)}$, and $k_{\delta}^{(f)} $ are valid covariance function with $\{\btheta_{f_x}, \btheta_{f_y}, \btheta_{f_\delta} \}$ denoting the corresponding hyperparameters.
%is also implemented.
These hyperparameters could be learned via maximum-likelihood estimation as in equation~\eqref{eq:sgp likelihood} using input date $\{\X^{(f)}, \Y^{(f-1)}\}$ and output data $\Y^{(f)}$.
%using available design input and related fidelity data. 
This method required estimation of $(l+3)$ hyperparameters with a ARD kernel for each fidelity model.

%\textbf{[!!discussion of this formulation] It is also pointed out that when using a stationary kernel, this leads to an Markov property that we can learn nothing more about $g^{(f)}(\x)$ form any other model output $g^{(f-1)}(\x)$ for $\x \neq \x'$.}

Despite being much more efficient than the full deep GP with variational inference, this GP autoregressive model does not naturally extend to multivariate cases, especially those of very high dimension. 
%First, the correlation function will need to encode the output correlation using a more complicated kernel function such as $k^{(f)}\left(\x, \x', \y(\x), \y(\x'), i,j \right)$, where $i$ and $j$ denotes the $i-th$ and $j-th$ output.
First, it consider the outputs in each layer as independent (given the inputs) and it is unclear how to model the strong output correlations, which is crucial for learning with a small set of training examples. 
%While we can extend Equation\eqref{eq:deep gp} to a standard deep GP that samples multiple functions in each layer, it feeds all the outputs into the next layer and hence is not scalable to a large number of outputs, say, millions. 
Second, the deep kernel function $k_y^{(f)}$ in equation~\eqref{eq:deep sgp} requires $d$ hyperparameters to be optimized using the default ARD kernel.
This is practical impossible with our problem where $d$ is of the scale of 1 billion.

\subsection{Deep Linear Model of Coregionalization}
In order to model high dimensional outputs, we borrow the classic multiple output Gaussian process framework, Linear Model of Coregionalization (LMC)\citep{matheron1982pour}, to represent the $f$ fidelity high dimensional output as,
%which assumes a linear low-rank structure for the high dimensional output as,
%The LMC represents the a multiple output as a linear combination of $R$ latent process,
\begin{equation} \label{eq:lmc}
\y^{(f)}(\x) = \sum_{r=1}^R \b^{(f)}_r z^{(f)}_r(\x) = \B^{(f)} \z^{(f)}(\x). 
\end{equation}
In this formulation, $\b^{(f)}_r \in \mathbb{R}^d$ represents a base vector with $\B^{(f)} = [\b^{(f)}_1,\dots,\b^{(f)}_R]$ being the collection of bases; $\z^{(f)}(\x) = [\z^{(f)}_1(\x),\dots,\z^{(f)}_R(\x)]^T$ is the collection of latent processes.
It is also assumed that the latent processes are independent, i.e., $\cov( z^{(f)}_r(\x), z^{(f)}_{r'}(\x')) = 0$ for $r \neq r'$. 
Due the linear nature, we have,
%\textbf{[It is often assumed that that bases are orthogonal, i.e., $(\b^{(F)}_r)^T \b^{(F)}_{r'} = 0 $ for $r \neq r'$.]}
%This formulation allows us to seek a low-rank model approximation for very large dimensional output by decomposing the output correlation through $R$ latent process.
%A large value of $R$ will....
%\textbf{[discussion of B and z(x) and some review here]}

%If the latent processes are independent, i.e., $\cov(z_r(\x), z_{r'}(\x)) = 0 $ if $r \neq r'$,
%given two input parameters, the multiple output correlation matrix can be expressed as,
%\begin{equation}
%\K^{(F)}_m = \sum_{r=1}^R \b^{(F)}_r {\b^{(F)}_r}^T k^{(F)}_r(\x,\x') = \B^{(F)} \k^{(F)}(\x,\x') {\B^{(F)}}^T
%\end{equation}
%where $\K^{(F)}_m$ denote the correlation matrix of the outputs and $k^{(F)}_r(\x,\x')$ is the input covariance $r$. 

\begin{lemma}
\label{lemma1}
A LMC model assumes a multivariate Gaussian prior:
\begin{equation*}
\begin{aligned}
 \y^{(f)}(\x) &= \mathcal{N}(\0, \B^{(f)} \K^{(f)}(\x,\x') {\B^{(f)}}^T )\\
\K^{(f)}(\x,\x') &= \diag\left(k^{(f)}_1(\x,\x'),\dots,k^{(f)}_R(\x,\x') \right).
\end{aligned}
\end{equation*}
\end{lemma}
We leave the proof in the Appendix. This property allow us to substitute the LMC in the GP autoregressive model without adding more assumption and to derive the following:
\begin{lemma}
\label{lemma2}
	With the LMC representation, the deep kernel always has a equivalent compact kernel function based on previous latent process posterior,
	\[	k^{(f)}\left(\x, \x', \y_*^{(f-1)}(\x), \y_*^{(f-1)}(\x')\right) = \hat{k}^{(f)}\left(\x, \x', \z_*^{(f-1)}(\x), \z_*^{(f-1)}(\x)\right). \]
\end{lemma}

With lemma \ref{lemma1} and \ref{lemma2}, we now derive a low-rank equivalent GP autoregressive model: 
\begin{prop}
	If each fidelity date admits a LMC representation, there exist a low-rank independent deep structure that fully capture the information of data and uncertainty,
	\[
	z_r^{(f)}(\x) = \widehat{g}_r^{(f)}(\x, \z_*^{(f-1)}(\x)).
	\]
\end{prop}
Now the high dimensional deep GP is disentangled into multiple low dimensional univariate GPs that are free from massive hyperparameters and complex multivariate model.

\subsection{Residual principal bases}
The challenge is the choice of low-rank $R$ and the construction of bases $\B^{(f)}$ for each fidelity data.
If we set $R=1$ for each fidelity data, we recover the \textit{intrinsic coregionalization model} (ICM)~\citep{goovaerts1997geostatistics} where an efficient Kronecker structure could be utilized to speed up computation. But the model capacity can be quite limited due to the over simplified latent process. A larger $R$ enables us to model outputs with different characteristics~\citep{alvarez2012kernels} with the cost of more hyperparameters to infer.
The output correlation can be indirectly modeled using a full-rank or low-rank Cholesky decomposition to allow flexible output correlation\citep{bonilla2008multi}.
The number of hyperprameter to infer for the aforementioned methods is proportional to $d \times R$. They are thus not suitable our application considering the large $d$ and the scarce high fidelity data. 
%These aforementioned methods all require joint learning $d\times R$ hyperprameter to encode the spatial correlation. This can be problematic for our application considering the large $d$ and the scarce high fidelity data.
Since the simulation outputs are always complete and can be efficiently represented via principal components~\citep{ramsey1997functional},
\citet{higdon2008computer} suggests using the principal components as the bases. 
More specifically, after standardize the data, singular value decomposition (SVD) is applied to $\Y^{(f)}$. The first $R$ left singular vectors is then used as the base matrix $\B^{(f)}$.
%for $\Y^{(f)}$, we can first standardize the result in a $N_f \times d$ matrix $\widetilde{\Y}^{(f)}$ and obtain the bases matrix $\B$ by using the first $R$ principal components of $\widetilde{\Y}^{(f)}$.
Another benefit of \citep{higdon2008computer} is a heuristic method to choose the number of bases by choosing $R$ such that at least $90\%$ of the variance of the results is explained. 
It is reported that the components which explains minor trend of the variation do not add to the predictive ability of the GP model.

Despite this approach works well for many single-fidelity applications~\citep{higdon2008computer,zhe2019scalable}, direct implement is problematic for our applications.
%First, for high fidelity data, $\Y^{(f)}$ where $f$ is large, the data is scarce.
First, the principal components are essentially based on the empirical covariance matrix given data $\Y^{(f)}$. 
We are often provided with a limited number of high-fidelity sample. The empirical covariance matrix is a very rough approximation to the real one and the resulting principal components are consequently inaccurate.
Second, even provided that we are always given enough samples to explore the output correlation at each fidelity level, direct implementation of \citet{higdon2008computer} is of low efficiency.
According to our experiment, when directly implementing SVD to each fidelity data, the dominant components (the low-frequency components) and corresponding coefficients of each fidelity level are very similar.
This means propagating these coefficients in the latent process can be of low efficiency.
Instead, we can limit the information passing down the model by only look at the added information.
%To take the advantage of such nature, rather than applying \citet{higdon2008computer} to each fidelity data, we apply it to the residual the information. 
%To avoid this issues, we introduce a residual structure. 
Specifically, we specify,
\begin{equation}
\begin{cases}
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) \;\; &\mathrm{for} \; f = 1 \\
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) + \y^{(f-1)}(\x)  \;\; &\mathrm{for} \; f \geq 2 \\
\end{cases}
\end{equation}
We call this formulation \textit{residual principal component analysis} since that for each fidelity data, we only need to learn the residual (additional) information compared with the previous fidelity model. 
%This formulation means that each fidelity model only need to learn the additional information compared with the previous fidelity model. 
%The lower fidelity models provide the low frequency signals while the higher fidelity models offer detailed information for the system.
Except for efficiency, another advantages of this approach is that the prediction posterior for high-fidelity results are decomposed into a tractable additive structure. We can easily identify where the main uncertainty is from and adjust the model accordingly.
%
%An other benefit of this formulation is that, unlike traditional deep GPs, where the predictive uncertainty is propagated and accumulating, our our method admit a additive uncertainty structure where the uncertainty for each 
Practical implementation of the residual principal component analysis can be done 
%by approximating the residual covariance matrix using empirical data and 
through SVD, which is more numerical stable than direct eigendecomposition on the empirical covariance matrix, as in Algorithm~\ref{algo:rpca}.
%\begin{equation}
%\B^{(f)} = PCA(\Y^{(f)} - \Y^{(f-1)}) = \cov[\y^{(f)}(\x) - \y^{(f-1)}(\x)]
%\end{equation}
%\begin{equation}
%\var[\y^{(f)}(\x) - \y^{(f-1)}(\x)] = \EE[\y^{(f)}(\x) - \y^{(f-1)}(\x) -]
%\end{equation}
\begin{algorithm}[h]
	\caption{Residual-PCA}
	\label{algo:rpca}
	\begin{algorithmic}[1]
		\Require
		multi-fidelity multivariate data $\{\X^{(f)},\Y^{(f)} \}_{f=1}^F$
		\Ensure
		Residual bases $\{\B^{(f)}\}_{f=1}^F$;
		Residual coefficients $\{\Z^{(f)}\}_{f=1}^F$;
		\State $\B^{(1)} = \mathrm{SVD}({\Y}^{(1)})$; \; $\Z^{(1)} = {\Y}^{(1)} {\B^{(1)}}^T$
		\For{each $ f \in [2,F]$}
		\State Achieve residual information $\widetilde{\Y}^{(f)} = \Y^{(f)} - \Y^{(f-1)}_{\e_{f-1},:} $
%		\State Standardize  $\widetilde{\Y}$
		\State Achieve residual base $\B^{(f)} = \mathrm{SVD}(\widetilde{\Y}^{(f)})$
		\State Achieve residual coefficient $\Z^{(f)} = \widetilde{\Y}^{(f)} {\B^{(f)}}^T$
		\EndFor
		\label{code:recentEnd}
	\end{algorithmic}
\end{algorithm}

\subsection{Prediction and uncertainty propagation}
Due to the intractability of a deep GP structure, except for the latent posterior corresponding to the lowest fidelity $\z^{(1)}(\x_*)$, the predictive posterior for the latent process is,
\begin{equation}
\label{eq:dgp posterior}
p(\z_*^{(f)}(\x_*)) = \int g^{(f)}(\x_*, \z_*^{(f-1)}) p(\z_*^{(f-1)}) d \z_*^{(f-1)},
\end{equation}
which is no longer a Gaussian and this integral is intractable.
We can use either Monte Carlo integration to derive the latent posterior or 
apply a Gaussian approximation of each latent posterior as in \citep{perdikaris2017nonlinear,girard2003gaussian}.
%and is difficult to solve for large $R$
%But it could be solved using Monte Carlo integration.
%The field posterior is an affine transformation from the latent process and normally has a simple close form solution once we know the distribution of $\z_*^{(f)}(\x_*)$.
%The field posterior is an affine transformation from the latent process and the first two  1st and 2nd order moment have a close form.
The mean field prediction have a analytical form as,
\begin{equation}
\label{eq:dgp fmean}
\EE[\y_*^{(F)}(\x_*)] = \sum_{f=1}^F \B^{(f)}\EE[\z_*^{(f)}(\x_*)].
\end{equation}
For the predictive field variance, we can derive,
\begin{equation}
\begin{aligned}
\label{eq:dgp fvar}
& \var[\y_*^{(F)}(\x_*)] = \B^{(1)}\var[\z_*^{(1)}(\x_*)]{\B^{(1)}}^T \\
&+ \sum_{f=2}^F \left( \B^{(f)}\var[\z_*^{(f)}(\x_*)]{\B^{(f)}}^T 
 - 2\B^{(f)}\cov[\z_*^{(f)}(\x_*),\z_*^{(f-1)}(\x_*)]{\B^{(f-1)}}^T \right)
\end{aligned}
\end{equation}
where $\cov[\z_*^{(f)}(\x_*),\z_*^{(f-1)}(\x_*)]$ is the approximated covariance between $\z_*^{(f)}(\x_*)$ and $\z_*^{(f-1)}(\x_*)$.
 
%\begin{corol}
%	Given 1st and 2nd order moment of $\z_*^{(f)}(\x_*)$,
%	% i.e., $\EE(\z_*^{(f)}(\x_*)) = \pmb\mu$ and $\cov(\z_*^{(f)}(\x_*)) = \bSigma^{(f)}$, 
%	the 1st and 2nd order moment of the field prediction has a close form as,
%	\begin{equation*}
%	\begin{aligned}
%		\EE(\y_*^{(F)}(\x_*)) &= \sum_{f=1}^F \B^{(f)}\EE(\z_*^{(f)}(\x_*)); \;\;\;\;\\
%		 \var(\y_*^{(F)}(\x_*)) &= \B^{(f)}\EE(\z_*^{(f)}(\x_*)) {\B^{(f)}}^T
%	\end{aligned}
%	\end{equation*}
%\end{corol}
%Further more, if $\z_*^{(f)}$ could be approximate using a multivariate Gaussian distribution $\z_*^{(f)}(\x_*)  \sim \N\left(\pmb\mu^{(f)}, \bSigma^{(f)} \right)$, then the output field $\y_*^{(f)}(\x_*) \sim \N\left(\B^{(f)}\pmb\mu^{(f)}, \B^{(f)}\bSigma^{(f)} {\B^{(f)}}^T \right)$ is also a multivariate Gaussian.

\subsection{Implementation and model complexity}
In this section we review the workflow of our model.
1). To build a surrogate model, We need to first collect different fidelity data from a simulator at design inputs $\X$. To better explore the response surface, we use a sobol sequence~\citep{sobol1976uniformly} to generate the design points. For $f$ fidelity data, we choose the first $N_f$ design points of $\X$ to generate the corresponding outputs.
2). We then apply Algorithm~\ref{algo:rpca} to get the residual bases $\{\B^{(f)}\}_{f=1}^F$ and coefficient $\{\Z^{(f)}\}_{f=1}^F$. For the choice of the preserved number of base, we can set a variance shareholder as in \citep{higdon2008computer}. 
3). For each pair of $\{ (\Z^{(f-1)}_{e_f},\X_{e_f}),\Z^{(f)}\}$, train independent GP by maximizing the marginal log-likelihood of equation \eqref{eq:sgp likelihood}.
In this work, we use a L-BFGS-B for the optimization.  Though complete independent training can improve model flexibility, we found that conditional independent training, i.e., sharing the hyperparameter $\btheta^{(f)}$ for the independent latent GP produce more stable results with very little loss of model accuracy. With the conditional independent assumption, the complexity of each GP is $\Ocal(N_f^3)$. For large number of observations, sparse GPs~\citep{snelson2005sparse} could applied to reduce the large computational complexity.
4). Once all the fidelity GP models are trained, we first calculate each latent posterior using equation \eqref{eq:dgp posterior} and derive the high dimensional posterior using equation~\ref{eq:dgp fmean} and \ref{eq:dgp fvar}.

%For high dimensional latent process, we can also apply a Gaussian approximation of all the residual posterior which yields closed form posterior\citep{perdikaris2017nonlinear,girard2003gaussian}. The first two moment of the field outputs can be derived using equation\eqref{label} once given the first two moment of the latent posterior.

%The simplest way is to specified $B$
%Implementation using PCA.
%Implementation of LMC can be done based on different way on defining the bases.
%For our application where the $d$ is very large, learning the bases jointly can be very difficult. Instead, we can use the PCA base from the data to construct the bases\citep{higdon2008computer}. 







==> model_v2.tex <==
\section{Statement of the problem}\label{emulate}
Consider a parameterized nonlinear system of steady-state or transient PDEs of arbitrary order for dependent variables (scalar fields) $u(\x,\s ,t)$, where $\x\in \mathbb{R}^l$ is a vector that parameterizes the PDEs, $\s$ and $t$ denotes spatial and temporal index.
% To give a concrete example, the $u_i$, $i=1,\hdots,4$, could refer to velocity components (say $i=1,2,3$) and pressure ($i=4)$ in a fluid flow model. 
The PDEs can be fully nonlinear and parameterized in an arbitrary fashion (including the initial and boundary conditions); it is also assumed to be well-posed (\ie solutions always exist and are unique) for the range of values of $\x$ considered.

The quantities of interest is the function $u(\x,\s,t)$ in given range of $\x$.
Direct approximation of this function is difficult due to the amount of samples we need to cover the response surface for such a high dimensional space~\citep{higdon2008computer}.
Instead, we can record values at specified (fixed) spatial locations, $\s_i$, $i=1,\dots,d_s$, and temporal locations, $t_i$, $i=1,\dots,d_t$.
For different inputs parameters $\x_i\in \mathbb{R}^l$, the  outputs of the simulator are represented as vectors: $\y^{(F)}_i = \y^{(F)}(\x_i) = (u(\x_i,\s_1,t_1),...,u(\x_i,\s_{d_s},t_{d_t}))^T \in \mathbb{R}^d$, where $d=d_s\times d_t$. 
Here, we use the superscript ${(F)}$ to denote that resulting vector is from an accurate, high-fidelity simulation.
%As is suggested in \citep{higdon2008computer},
The value at a different spatial-temporal locations can be achieved easily through interpolation provided that the spatial-temporal fixed points are dense enough; interpolations in this case come with ignorable extra computational effort~\citep{higdon2008computer}.
With the preceding process, the simulation is now treated as a mapping from $\mathbb{R}^l$ to $\mathbb{R}^d$, where $d$ is extremely large.
The goal of a data-driven surrogate is to approximate the mapping given training set $\mathcal{D} = \{\X, \Y^{(F)}\}$, where $\X = [\x_1,\ldots,\x_N]^T$ and $\Y^{(F)} = [\y^{(F)}_1,\ldots,\y^{(F)}_N]^T$.
%where $\y^{(F)}_i$ denotes the finest fidelity data that are very close to the ground truth value and the corresponding inputs $\x_i$ are referred to as {\/\it design inputs\/}. 
Provided enough number of samples to cover the response surface, we can approximate the mapping accurately.

As discussed in the introduction, we intend to avoid relying on only high-fidelity data. 
%In practice, getting accurate high fidelity data is computational expensive; it is impractical to get enough samples to cover the response surface of our interest.
The low-fidelity data can be easily obtain cheaply by reducing the fidelity setting (\eg the number of nodes of a discretization mesh and the order of basis functions of the finite element method) of a simulator.
In general, we can run a simulation at different fidelity settings to obtain 
multi-fidelity dataset $\{\X^{(f)}, \Y^{(f)}\}_{f=1}^F$, where $\Y^{(f)}$ is a $N_f\times d$ matrix for observations at fidelity $f$ with $\X^{(f)}$ being a $N_f\times l$ matrix for the corresponding inputs.
We use $f=F$ to denote the highest fidelity and $f=1$ the lowest.
%It is, however, practically easy to compromise the accuracy by ruining a simulator, given input $\x_i$ in a lower fidelity setting to collect cheaper but less accurate observation $\y_i^{(F-1)}$ and even cheaper observation $\y_i^{(F-2)}$.
%We denote the all fidelity data by 
Following the common setting for multi-fidelity data in~\citep{perdikaris2017nonlinear,cutajar2019deep}, we also require that the training inputs of fidelity $f$ is a subset the previous fidelity $f-1$, .i.e, $\X^{(f)} \subset \X^{(f-1)}$. For convenience, 
% It is obvious that for $f\geq2$, $\X^{(f)} \subset \X^{(1)}$.
we introduce the index notation $\e$ to extract raws form a standard matrix such that $\X^{(f)} = \X_{\e_f,:}$, where $\e_f$ indicating the subset indexes for fidelity data $f$ and $\X$ contains all candidates.
Our goal of surrogate model becomes: given multi-fidelity data $\{\X^{(f)}, \Y^{(f)}\}_{f=1}^F$, how to efficiently approximate the mapping between $\x$ and $\y^{(F)}$.


%It is assumed for now that a single output $\mbox{\textbf{\textit{y}}}$ (derived from a single scalar field $u({\textbf{\textit{x}}};{\pmb{\xi}})$) is the target for emulation. 
%
%From the preceding discussion, the simulator can be considered as a mapping $\pmb{\eta}:{\cal X}\rightarrow {\cal M}$ (assumed to be injective), where ${\cal M}\subset \mathbb{R}^d$ is the permissible output space (response surface) and ${\cal X} \subset \mathbb{R}^l$ is the permissible input space. That is, $\pmb{\eta}(\pmb{\xi})= \mbox{\textbf{\textit{y}}}=(u(\textbf{\textit{x}}^{(1)};\pmb{\xi}),\dots,u(\textbf{\textit{x}}^{(d)};\pmb{\xi}))^T$ for an arbitrary input $\pmb{\xi}$. 

%To infer outputs of the simulator at new inputs, Conti and O'Hagan~\cite{Conti2010} took the approach of placing a $d$-dimensional GP prior over $\pmb{\eta}$, indexed by $\pmb{\xi}$.  Effectively, the same assumption was made by Higdon {\/\em et al.\/}~\cite{Higdon} but in that case the outputs were a linear combination of PCA basis vectors with coefficients  treated as independent univariate GPs indexed by $\pmb{\xi}$. In this paper, a similar approach is adopted but rather than using PCA coefficients  we place GP priors over coefficients of a reduced-dimensional approximation of  points in ${\cal M}$, obtained by manifold learning methods. We assume that  ${\cal M}$ is a smooth manifold in $\mathbb{R}^d$. The high dimension $d$ of the output space  and the inability of linear dimensionality reduction methods such as PCA to capture complex response surfaces  is the motivation for our approach. 

\section{Model Formulation}
%problem definiteion --- deep gp (with introduction of sgp) --- lmc model --- deep lmc model 

\subsection{Univariate Gaussian Process}
\label{sec:sgp}
We first review the GP regression for learning a univariate function using a fine fidelity dataset $\Dcal = \{\X, \Y^{(F)}\}$.
The quantity of interest is assumed univariate, i.e., $d=1$. We use $y^{(F)}_i$ to distinct a univariate observation from a multivariate one $\y^{(F)}_i$.
%where each $\x_i$ is a $l$ dimensional input vector, and $y^{(F)}_i$ the observed scalar output, we aim to learn a function $f: \mathbb{R}^p \rightarrow \mathbb{R}$. 
A GP assumes the finite set of function values on $\X = [\x_1, \ldots, \x_N]^\top$, namely $\y^{(F)} = [y^{(F)}_1, \ldots, y^{(F)}_N]^\top$, follows a multivariate Gaussian distribution, 
$p(\y^{(F)} | \X) = \N(\y^{(F)} | \m, \K + \tau^{-1} \I)$.
Here $\m = [m(\x_1), \ldots, m(\x_n)]^\top$ is the mean function that is usually set to $\0$ after centering $\Y^{(F)}$ and 
$\tau$ is the inverse noise variance, which accounts for model inadequacies and numerical error~\citep{kennedy2001bayesian,rasmussen2003gaussian}.
$\K$ is the covariance matrix with elements $[\K]_{ij} = k(\x_i, \x_j)$, where $k(\x_i, \x_j)$ is a kernel function for the corresponding inputs.
Choosing the right kernel function for a specific application is nontrivial. 
When there is no prior knowledge to guide the choice, the automatic relevance deterrence (ARD) kernel \citep{rasmussen2003gaussian},
\begin{equation}
	k(\x_i, \x_j) = \theta_0 \exp\left(-(\x_i-\x_j) \diag(\theta_1,\ldots,\theta_l) (\x_i-\x_j)^T \right),
\end{equation}
is normally utilized. The ARD kernel can freely capture the individual influence of each input parameter on the output results.
The hyperparameters $\{\tau,\theta_0, \ldots, \theta_l\}$ can be estimated by maximizing  the  marginal likelihood of the GP regression,
\begin{equation}
\label{eq:sgp likelihood}
\Lcal = \frac{1}{2} \ln|\K| - \frac{1}{2}{\y^{(F)}}^T \K^{-1} \y^{(F)} - \frac{N}{2} \ln(2\pi).
\end{equation}
The main computational cost is the inversion of $\K$, which is $\Ocal(N^3)$ and $\Ocal(N^2)$ time and space complexity, respectively.
Given a new input $\x_*$, we can now derive its posterior using a conditional Gaussian distribution,
\begin{equation}
\label{eq:sgp}
\begin{aligned}
 p\big(y^{(F)}_*|\x_*, \X,\y\big) &= \N\left(y^{(F)}_* | \mu(\x_*), v(\x_*)\right) \\
 \mu(\x_*) &= \k_{*}^\top (\K + \tau^{-1} \I)^{-1}\y^{(F)} \\
 v(\x_*) &= k(\x_*, \x_*) - \k_{*}^\top(\K + \tau^{-1}\I)^{-1}\k_{*},
\end{aligned}
\end{equation}
where, $\k_{*} = [k(\x_*, \x_1), \ldots, k(\x_*, \x_{N_F})]^\top$ is the vector of covariance between $\x_*$ and $\X$. 

%The inference of the GP regression is to estimate the covariance (or kernel) parameters (\eg $\{\theta_0, \ldots, \theta_l\}$ in the ARD  kernel) and the inverse noise variance $\tau$ that best explain the observed data $\Dcal$.
%We can optimize these hyperparameters by maximizing  the  marginal likelihood likelihood,
%\begin{equation}
%\label{eq:sgp likelihood}
%	\Lcal = \frac{1}{2} \ln|\K| - \frac{1}{2}\Y^T \K^{-1} \Y - \frac{N}{2} \ln(2\pi).
%\end{equation}
%The main computational cost is the inversion of $\K$, which takes $\Ocal(N^3)$ and $\Ocal(N^2)$ time and space complexity, respectively.

\subsection{Deep Gaussian Process Autoregression}
Now, let us incorporate the multi-fidelity univariate data,
\ie $\{\X^{(f)},\Y^{(f)}\}_{f=1}^F$ where $\Y^{(f)} = [y^{(f)}_1,\ldots,y^{(f)}_{N_f}]^T $ is a collection of samples at fidelity $f$.
%First, let consider the traditional GP for multi-fidelity data where the quantity of interest is a univariate, i.e., $d=1$ for our problem. We use $y$ to distinct the univariate observations from a multivariate one $\y$.
The general autoregressive formulation for multi-fidelity data is,
% data put forward by \citep{perdikaris2017nonlinear} is
\begin{equation}
y^{(f)}(\x) = g^{(f)}\left(y^{(f-1)}(\x)\right) + \epsilon^{(f)}(\x),
\end{equation}
where $g^{(f)}(y^{(f-1)}(\x))$ is an arbitrary function that maps the low fidelity result to the high fidelity one and $\epsilon^{(f)}(\x)$ captures the model inadequacies and numerical error.
If we assume a simple linear form for the mapping, i.e.,  $g^{(f)}(\y^{(f-1)}(\x)) = c \cdot \y^{(f-1)}(\x)$, we recover the classic autoregressive model~\citep{kennedy2000predicting}.
This method is further improved by \citet{le2013multi} using a deterministic parametric form of $g^{(f)}$ and an efficient numerical scheme to reduce the computational cost. 
Despite being successful to deal with some problems, 
this parametric approach does not generalize well due to the difficulty of model selections and the demand for large training datasets~\citep{perdikaris2017nonlinear}.
To resolve this issue, a Bayesian non-parametric treatment can be implemented by placing a GP prior over the function $g^{(f)}$.
This is also known as the \textit{deep GP}~\citep{damianou2013deep}.
Although being capable of modeling complex problem, deep GP is infamous for its intractability. They requires computationally expensive variational approximation for model training and thus quickly become infeasible for multi-fidelity simulation problems.
\citet{perdikaris2017nonlinear} put forward an GP based nonlinear autoregressive scheme with an additive structure,
\begin{equation} \label{eq:deep gp}
y^{(f)}(\x) = g^{(f)}\left(\x, y_*^{(f-1)}(\x)\right),
\end{equation}
where the error term is absorbed into $g^{(f)}(\x)$. This formulation specifies that $y^{(f)}(\x)$ is a GP posterior given the previous fidelity observations and the model inputs.
%which is effective for the multi-fidelity problem.
To better reflect the autoregressive nature, \citet{perdikaris2017nonlinear} suggested a covariance function that decomposes as
\begin{equation}
\label{eq:deep gp kernel}
\begin{aligned}
&k^{(f)}\left(\x, \x', y_*^{(f-1)}(\x), y_*^{(f-1)}(\x)\right)\\ &=  k_x^{(f)}(\x, \x'; \btheta_{fx} ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x), y_*^{(f-1)}(\x'); \btheta_{fy} ) +k_{\delta}^{(f)}(\x, \x'; \btheta_{f\delta}),
\end{aligned}
\end{equation}
where $k_x^{(f)}$, $k_y^{(f)}$, and $k_{\delta}^{(f)} $ are valid covariance function with $\{\btheta_{f_x}, \btheta_{f_y}, \btheta_{f_\delta} \}$ denoting the corresponding hyperparameters.
%is also implemented.
These hyperparameters could be learned via maximum-likelihood estimation as in Eq.~\eqref{eq:sgp likelihood} using input date $\{\X^{(f)}, \Y^{(f-1)}\}$ and output data $\Y^{(f)}$.
%using available design input and related fidelity data. 
This method requires estimation of $(l+3)$ hyperparameters with a ARD kernel for each fidelity model.

Despite being much more efficient than the full deep GP with variational inference, this GP autoregressive model does not naturally extend to multivariate cases, especially to those of very high dimension. 
%First, the correlation function will need to encode the output correlation using a more complicated kernel function such as $k^{(f)}\left(\x, \x', \y(\x), \y(\x'), i,j \right)$, where $i$ and $j$ denotes the $i-th$ and $j-th$ output.
First, it consider the outputs in each layer as independent (given the inputs) and it is unclear how to model the strong output correlations, which is crucial for learning with a small set of training examples. 
%While we can extend Equation\eqref{eq:deep gp} to a standard deep GP that samples multiple functions in each layer, it feeds all the outputs into the next layer and hence is not scalable to a large number of outputs, say, millions. 
Second, when using an anisotropic kernel such as the ARD, the deep kernel function $k_y^{(f)}$ in Eq.~\eqref{eq:deep gp} requires $d$ hyperparameters to be optimized .
This is practical impossible with our problem where $d$ can scale up to 1 billion.

\subsection{Deep Linear Model of Coregionalization}
In order to model the high dimensional output correlations within limited computational resources, we borrow the classic multiple output Gaussian process framework---Linear Model of Coregionalization (LMC)~\citep{matheron1982pour}---to decompose the $f$ fidelity high dimensional output,
%which assumes a linear low-rank structure for the high dimensional output as,
%The LMC represents the a multiple output as a linear combination of $R$ latent process,
\begin{equation} \label{eq:lmc}
\y^{(f)}(\x) = \sum_{r=1}^{R_f} \b^{(f)}_r z^{(f)}_r(\x) = \B^{(f)} \z^{(f)}(\x). 
\end{equation}
In this formulation, 
$\B^{(f)} = [\b^{(f)}_1,\dots,\b^{(f)}_{R_f}]$ is the collection of bases $\b^{(f)}_r \in \mathbb{R}^d$; $\z^{(f)}(\x) = [\z^{(f)}_1(\x),\dots,\z^{(f)}_{R_f}(\x)]^T$ is the collection of corresponding latent processes.
It is assumed that the latent processes are independent, i.e., $\cov( z^{(f)}_r(\x), z^{(f)}_{r'}(\x')) = 0$ for $r \neq r'$ and the bases are orthogonal.
The LMC model essentially assumes several independent latent processes to fully characterize the data variability. It is shown particularly efficient for the simulation-type problems\citep{higdon2008computer,zhe2019scalable}.
Assuming $\{\B^{(f)}\}_{f=1}^F$ is known, we can substitute Eq.~\eqref{eq:lmc} into Eq.~\eqref{eq:deep gp} to derive the deep latent process for the LMC model,
\begin{equation}
\begin{aligned}
\B^{(f)} \z^{(f)}(\x) & = \g^{(f)}\left(\x, \B^{(f-1)} \z_*^{(f-1)}(\x)\right),\\
\z^{(f)}(\x) & = {\B^{(f)}}^T \g^{(f)}\left(\x, \B^{(f-1)} \z_*^{(f-1)}(\x)\right)\\
\z^{(f)}(\x) & = \hat{\g}^{(f)}\left(\x,\z_*^{(f-1)}(\x)\right),\\
\end{aligned}
\label{eq:deep lmc1}
\end{equation}
where $\hat{\g}^{(f)}$ is the composite function absorbing $\B^{(f)}$ and $\B^{(f-1)}$ into the multivariate mapping $\g^{(f)}$.
%Generally, $\hat{\g}^{(f)}$ is not necessary a multivariate GP given that $\g^{(f)}$ is a multivariate GP. Nevertheless, we can show that for a multivariate GP with the commonly assumed separable structure, $\hat{\g}^{(f)}$ is a Gaussian 
\begin{theorem}
\label{THEMTEM1}
If the high dimensional GP autoregression $\g^{(f)}(\x,\y_*^{(f-1)}(\x))$ admits a separable structure, it must be able to be decomposed into several independent univariate GPs $g_r^{(f)}(\x,\z_*^{(f-1)}(\x))$ .


\end{theorem}
We leave the proof in Appendix \ref{ap:proof t1}. In cases where the original high-dimensional GP $\g^{(f)}$ does not have a separable structure, without loss of generality, we can still place a Gaussian prior over $\hat{\g}^{(f)}$ as an non-parametric Bayesian regression.
% assume a multivariate GP as in the univariate deep GP and place a Gaussian prior over 
%
%The only difference form the univariate case is that this GP is multivariate. However, 
Since the LMC requires the latent process to be independent from each other, Eq.~\eqref{eq:deep lmc1} further decomposes as
\begin{equation}
z_r^{(f)}(\x) = \hat{g}_r^{(f)}\left(\x,\z_*^{(f-1)}(\x)\right),
\end{equation}
where each $\hat{g}_r^{(f)}$ is an independent GP and could be modeled separately using the univeriate GP model introduced in section~\ref{sec:sgp}. 
Since we will have limited high-fidelity data, we adopt a conditional independent approach, \ie the latent processes are independent given the same hyperparameters. The marginal likelihood of the conditional independent latent process at fidelity $f$ is
\begin{equation}
\label{eq:cigp likelihood}
\Lcal_f = \frac{R_f}{2} \ln|\K_f| - \frac{R_f}{2}{\Z^{(f)}}^T \K_f^{-1} \Z^{(f)} - \frac{R_f N_f}{2} \ln(2\pi),
\end{equation}
where $[\K_f]_{ij} = k_f\left(\x_i,\z_*^{(f-1)}(\x_i),\x_j,\z_*^{(f-1)}(\x_j) \right)$ is the covariance matrix and $\Z^{(f)}=[\z(\x_1)^T,\ldots,\z(\x_{N_f})^T]^T$ is the collection of latent process coefficients.
The conditional independent assumption reduce the hyperparameters from $R_f(R_{f-1}+3)$ to $R_{f-1}+3$ and computation complexity from $\Ocal(R_f N_f^3)$ to $\Ocal(N_f^3)$ compared to the fully independent approach.
%\begin{lemma}
%\label{lemma1}
%A LMC model assumes a multivariate Gaussian prior:
%\begin{equation*}
%\begin{aligned}
% \y^{(f)}(\x) &= \mathcal{N}(\0, \B^{(f)} \K^{(f)}(\x,\x') {\B^{(f)}}^T )\\
%\K^{(f)}(\x,\x') &= \diag\left(k^{(f)}_1(\x,\x'),\dots,k^{(f)}_R(\x,\x') \right).
%\end{aligned}
%\end{equation*}
%\end{lemma}
%We leave the proof in the Appendix. This property allow us to substitute the LMC in the GP autoregressive model without adding more assumption and to derive the following:
%\begin{lemma}
%\label{lemma2}
%	With the LMC representation, the deep kernel always has a equivalent compact kernel function based on previous latent process posterior,
%	\[	k^{(f)}\left(\x, \x', \y_*^{(f-1)}(\x), \y_*^{(f-1)}(\x')\right) = \hat{k}^{(f)}\left(\x, \x', \z_*^{(f-1)}(\x), \z_*^{(f-1)}(\x)\right). \]
%\end{lemma}
%
%With lemma \ref{lemma1} and \ref{lemma2}, we now derive a low-rank equivalent GP autoregressive model: 
%\begin{prop}
%	If each fidelity date admits a LMC representation, there exist a low-rank independent deep structure that fully capture the information of data and uncertainty,
%	\[
%	z_r^{(f)}(\x) = \widehat{g}_r^{(f)}(\x, \z_*^{(f-1)}(\x)).
%	\]
%\end{prop}
%Now the high dimensional deep GP is disentangled into multiple low dimensional univariate GPs that are free from massive hyperparameters and complex multivariate model.

\subsection{Residual Principal Component Analysis}
The challenge for \ours is the choice of low-rank $R_f$ and the construction of bases $\B^{(f)}$ for each fidelity data.
If we set $R_f=1$ for each fidelity data, we recover the \textit{intrinsic coregionalization model} (ICM)~\citep{goovaerts1997geostatistics} where an efficient Kronecker structure could be utilized to speed up the computation. But the model capacity can be quite limited due to the over simplified latent process. A larger $R_f$ enables us to model outputs with different characteristics~\citep{alvarez2012kernels} with the cost of more hyperparameters to infer.
The output correlation can be indirectly modeled using a full-rank or low-rank Cholesky decomposition to allow flexible output correlations~\citep{bonilla2008multi}.
The number of hyperprameters to infer for the aforementioned methods are proportional to $d \times R_f$. They are thus not suitable our application considering the large $d$.
% and the scarce high fidelity data. 
%These aforementioned methods all require joint learning $d\times R$ hyperprameter to encode the spatial correlation. This can be problematic for our application considering the large $d$ and the scarce high fidelity data.
Since the simulation outputs are always complete and can be efficiently represented via principal components~\citep{ramsey1997functional},
\citet{higdon2008computer} suggested using the principal components as the bases. 
More specifically, after standardizing the data, singular value decomposition (SVD) is applied to $\Y^{(f)}$ and the first $R_f$ left singular vectors are then used as the bases $\B^{(f)}$.
%for $\Y^{(f)}$, we can first standardize the result in a $N_f \times d$ matrix $\widetilde{\Y}^{(f)}$ and obtain the bases matrix $\B$ by using the first $R$ principal components of $\widetilde{\Y}^{(f)}$.
Another benefit of this approach is a heuristic method to choose the number of bases by choosing $R_f$ such that at least $90\%$ of the variance of the output is covered by the bases. 
It is reported that the components which explains minor trend of the variation do not add to the predictive ability of the GP model.

Despite that this approach works well for many single-fidelity applications~\citep{higdon2008computer,zhe2019scalable}, a direct implement of this approach is problematic for our problem here.
%First, for high fidelity data, $\Y^{(f)}$ where $f$ is large, the data is scarce.
First, the principal components (the bases) are essentially based on the empirical covariance matrix given data $\Y^{(f)}$. 
Since we can only afford to have limited number of high-fidelity samples, the empirical covariance matrix is a very rough approximation to the real one and the resulting principal components are consequently inaccurate.
Second, even provided that we are always given enough samples to explore the output correlation at each fidelity level, direct implementation of \citet{higdon2008computer} is of low efficiency.
According to our experiments, when directly implementing SVD to each fidelity data, the dominant components (the low-frequency components) and their corresponding coefficients for each fidelity are very similar.
This means propagating these coefficients in the deep latent process is of low efficiency.
Instead, we can limit the information passing down the model and only model the updated (added) information.
%To take the advantage of such nature, rather than applying \citet{higdon2008computer} to each fidelity data, we apply it to the residual the information. 
%To avoid this issues, we introduce a residual structure. 
Specifically, we specify
\begin{equation}
\begin{cases}
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) \;\; &\mathrm{for} \; f = 1 \\
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) + \y^{(f-1)}(\x)  \;\; &\mathrm{for} \; f \geq 2. \\
\end{cases}
\end{equation}
In this formulation, each fidelity layer learns the residual (additional) information compared with the previous fidelity layer rather than the whole output information and thus we call this a \textit{residual deep structure} similar to the work of \citep{he2016deep}.
%We call this formulation \textit{residual principal component analysis} since that for each fidelity data, we only need to 
%This formulation means that each fidelity model only need to learn the additional information compared with the previous fidelity model. 
%The lower fidelity models provide the low frequency signals while the higher fidelity models offer detailed information for the system.
Except for efficiency, another advantages of this approach is that the predictive posterior for high-fidelity results naturally decompose into a additive structure. 
The additive structure can help us identify where the main uncertainty is from and adjust our model at each fidelity accordingly to reduce model uncertainty and improve model accuracy.
%
%An other benefit of this formulation is that, unlike traditional deep GPs, where the predictive uncertainty is propagated and accumulating, our our method admit a additive uncertainty structure where the uncertainty for each 

Inspired by the practical approach of \citep{higdon2008computer} to extract the bases, we introduce the \textit{residual principal component analysis} for our model. 
The method is a direct implementation of PCA on the residual information instead of the original data. We use SVD, which is more numerical stable than direct eigendecomposition on the empirical covariance matrix, to extract the eigenvectors. The detailed step of this method is presented in Algorithm~\ref{algo:rpca}.
%\begin{equation}
%\B^{(f)} = PCA(\Y^{(f)} - \Y^{(f-1)}) = \cov[\y^{(f)}(\x) - \y^{(f-1)}(\x)]
%\end{equation}
%\begin{equation}
%\var[\y^{(f)}(\x) - \y^{(f-1)}(\x)] = \EE[\y^{(f)}(\x) - \y^{(f-1)}(\x) -]
%\end{equation}
\begin{algorithm}[h]
	\caption{Residual-PCA}
	\label{algo:rpca}
	\begin{algorithmic}[1]
		\Require
		multi-fidelity multivariate data $\{\X^{(f)},\Y^{(f)} \}_{f=1}^F$ and index $\{\e_{f}\}_{f=1}^F$;
		\Ensure
		Residual bases $\{\B^{(f)}\}_{f=1}^F$;
		Residual coefficients $\{\Z^{(f)}\}_{f=1}^F$;
		\State $\B^{(1)} = \mathrm{SVD}({\Y}^{(1)})$; \; $\Z^{(1)} = {\Y}^{(1)} {\B^{(1)}}^T$
		\For{each $ f \in [2,F]$}
		\State Achieve residual information $\widetilde{\Y}^{(f)} = \Y^{(f)} - \Y^{(f-1)}_{\e_{f-1},:} $
%		\State Standardize  $\widetilde{\Y}$
		\State Achieve residual base $\B^{(f)} = \mathrm{SVD}(\widetilde{\Y}^{(f)})$
		\State Achieve residual coefficient $\Z^{(f)} =  {\B^{(f)}}^T \widetilde{\Y}^{(f)}$
		\EndFor
		\label{code:recentEnd}
	\end{algorithmic}
\end{algorithm}

\subsection{Prediction and uncertainty propagation}
Due to the intractability of a deep GP structure, except for the latent posterior $\z^{(1)}(\x)$ corresponding to the lowest fidelity $\y^{(1)}(\x)$, the predictive latent posterior for each fidelity is
\begin{equation}
\label{eq:dgp posterior}
\z_*^{(f)}(\x) = \int \g^{(f)}\left(\x, \z_*^{(f-1)}(\x) \right) p\left(\z_*^{(f-1)}(\x)\right) d \z_*^{(f-1)}(\x).
\end{equation}
%for $\space f=2,\ldots,F$.
This integral is intractable and the posterior is no longer a Gaussian. But we can approximate it numerically using sampling based methods. We can further reduce the complexity due to the independent assumption of the LMC; Eq.~\eqref{eq:dgp posterior} naturally decomposes as
\begin{equation}
\label{eq:dgp posterior decomp}
\z_{*}^{(f)}(\x) =  \prod_{k=1}^{R_f} \int g_k^{(f)}\left(\x, \z_*^{(f-1)}(\x) \right) \prod_{r=1}^{R_{f-1}} p(z_{*r}^{(f-1)}(\x)) d z_{*r}^{(f-1)}(\x).
\end{equation}
We can now easily implement Monte Carlo sampling methods to calculate the latent process posteriors. Another way to solve the intractable integral is to apply a Gaussian approximation of each latent posterior as in \citep{perdikaris2017nonlinear,girard2003gaussian}.
Once we obtain the approximated posterior, the first two order statistic admits a tractable solution due to the summation structure.
%For clarity, we organize all the bases and latent variable together, \ie 
%$\mathcal{B} = [\B^{(1)},\ldots,\B^{(F)}]$ 
%and $\mathcal{Z}(x) = [\z^{(1)}(\x),\ldots,\z^{(F)}(\x)]$.
%We can show that the first two statistical moments have a close form solution as,
\begin{lemma}
Given the posterior of the latent processes $\z^{(f)}(\x)$ and the bases $\B^{(f)}$, the mean and variance of the finest fidelity field $\y^{(F)}(\x)$ can be calculated as
\begin{equation}
\begin{aligned}
\EE[\y^{(F)}(\x)] &= \sum_{f=1}^F \B^{(f)}\EE[\z^{(f)}(\x)],\\
\var[\y^{(F)}(\x)] &= 
%\B^{(1)}\var[\z^{(1)}(\x)]{\B^{(1)}}^T \\
\sum_{f=1}^F \left( \B^{(f)}\var[\z^{(f)}(\x)]{\B^{(f)}}^T \right)\\
&- 2 \sum_{f\neq f'} \left(\B^{(f)}\cov[\z^{(f)}(\x),\z^{(f')}(\x)]{\B^{(f')}}^T \right).
\end{aligned}
\label{eq:y post}
\end{equation}
%$\var[\z^{(f)}(\x)]$ is the diagonal covariance matrix of the latent posterior for $f$ fidelity and $\cov[\z^{(f)}(\x),\z^{(f')}(\x)$ is the covariance matrix of $\z^{(f')}(\x)$ and $\z^{(f-1)}(\x)$. This covariance matrix could be calculated empirically using sampling methods. We leave the proof of this result in the Appendix.
\end{lemma}
%Once we obtain the empirical posterior, we can calculate the mean prediction as,
%\begin{equation}
%\label{eq:dgp fmean}
%\EE[\y^{(F)}(\x)] = \sum_{f=1}^F \B^{(f)}\EE[\z^{(f)}(\x)].
%\end{equation}
%Since the latent posteriors are unknown distribution, the predictive variance is also intractable. However, we if we use a sampling based method, we can calculate the predictive posterior for the highest fidelity as,
%\begin{equation}
%\begin{aligned}
%\label{eq:dgp fvar}
% \var[\y^{(F)}(\x)] &= 
%%\B^{(1)}\var[\z^{(1)}(\x)]{\B^{(1)}}^T \\
% \sum_{f=1}^F \left( \B^{(f)}\var[\z^{(f)}(\x)]{\B^{(f)}}^T \right)\\
% &- 2 \sum_{f=2}^F \left(\B^{(f)}\cov[\z^{(f)}(\x),\z^{(f-1)}(\x)]{\B^{(f-1)}}^T \right)
%\end{aligned}
%\end{equation}

$\var[\z^{(f)}(\x)]$ is the diagonal covariance matrix of the latent posterior for $f$ fidelity and $\cov[\z^{(f)}(\x),\z^{(f')}(\x)$ is the covariance matrix of $\z^{(f')}(\x)$ and $\z^{(f-1)}(\x)$. This covariance matrix could be calculated empirically using sampling methods. We leave the proof of this result in the Appendix.
%with the samples we get in the sampling process.
%\textbf{we leave the proof of the result in the appendix.}
 
%\begin{corol}
%	Given 1st and 2nd order moment of $\z_*^{(f)}(\x_*)$,
%	% i.e., $\EE(\z_*^{(f)}(\x_*)) = \pmb\mu$ and $\cov(\z_*^{(f)}(\x_*)) = \bSigma^{(f)}$, 
%	the 1st and 2nd order moment of the field prediction has a close form as,
%	\begin{equation*}
%	\begin{aligned}
%		\EE(\y_*^{(F)}(\x_*)) &= \sum_{f=1}^F \B^{(f)}\EE(\z_*^{(f)}(\x_*)); \;\;\;\;\\
%		 \var(\y_*^{(F)}(\x_*)) &= \B^{(f)}\EE(\z_*^{(f)}(\x_*)) {\B^{(f)}}^T
%	\end{aligned}
%	\end{equation*}
%\end{corol}
%Further more, if $\z_*^{(f)}$ could be approximate using a multivariate Gaussian distribution $\z_*^{(f)}(\x_*)  \sim \N\left(\pmb\mu^{(f)}, \bSigma^{(f)} \right)$, then the output field $\y_*^{(f)}(\x_*) \sim \N\left(\B^{(f)}\pmb\mu^{(f)}, \B^{(f)}\bSigma^{(f)} {\B^{(f)}}^T \right)$ is also a multivariate Gaussian.

\subsection{Implementation and model complexity}
Before we move to experiments, we review the workflow of our model and given some complexity analysis.
1). To build a surrogate model, We need to first collect different fidelity data from a simulator at design inputs $\X$. To better explore the response surface, we use a sobol sequence~\citep{sobol1976uniformly} to generate the design points. For $f$ fidelity data, we choose the first $N_f$ design points of $\X$ to generate the corresponding outputs $\Y^{(f)}$. The computational cost at this step depends on the simulator and the fidelity setting.
2). We then apply Algorithm~\ref{algo:rpca} to get the residual bases $\{\B^{(f)}\}_{f=1}^F$ and corresponding coefficients $\{\Z^{(f)}\}_{f=1}^F$. The computational cost for $f$ fidelity data is $\Ocal(\min(N_f^2 d,N_f d^2) )$. For the choice of low-rank $R_f$, we can set a variance shareholder as in \citep{higdon2008computer}.
In this work, we use a single low-rank for all fidelities, \ie $R=R_1=\ldots=R_F$.
When $R$ is a integer, it indicates the actual number of base each fidelity use, when $R$ is a decimal fraction, it indicates the minimum number of base to capture the ratio of given variance for each fidelity is used by the model.
3). For each pair of $\{ [\Z^{(f)},\Z^{(f-1)}_{e_f}],\X_{e_f})\}$, train $R_f$ independent GPs by maximizing the marginal log-likelihood of Eq.~\eqref{eq:sgp likelihood} when using fully independent GPs or Eq.~\eqref{eq:cigp likelihood} when using the conditional independent approach. The computational complexity, is $\Ocal(N_f^3 R_f)$ and $\Ocal(N_f^3)$, respectively for the two methods. 
In this work, we use a L-BFGS-B for the optimization. 
%Though complete independent training can improve model flexibility, we found that conditional independent training, i.e., sharing the hyperparameter $\btheta^{(f)}$ for the independent latent GP produce more stable results with very little loss of model accuracy. With the conditional independent assumption, the complexity of each GP is $\Ocal(N_f^3)$. 
For large number of observations, sparse GPs~\citep{snelson2005sparse} can be applied to reduce the large computational complexity.
4). Once all the fidelity GP models are trained, we first calculate each latent posterior using Eq.~\eqref{eq:dgp posterior} and then compute the mean and variance of the highest fidelity high-dimensional outputs using Eqs.~\ref{eq:y post}.

%For high dimensional latent process, we can also apply a Gaussian approximation of all the residual posterior which yields closed form posterior\citep{perdikaris2017nonlinear,girard2003gaussian}. The first two moment of the field outputs can be derived using equation\eqref{label} once given the first two moment of the latent posterior.

%The simplest way is to specified $B$
%Implementation using PCA.
%Implementation of LMC can be done based on different way on defining the bases.
%For our application where the $d$ is very large, learning the bases jointly can be very difficult. Instead, we can use the PCA base from the data to construct the bases\citep{higdon2008computer}. 







==> model_v3.tex <==
\section{Statement of the Problem}\label{emulate}
Consider a parameterized nonlinear system of steady-state or transient PDEs of arbitrary order for dependent variables (scalar fields) $u(\x,\s ,t)$, where $\x\in \mathbb{R}^l$ is a vector that parameterizes the PDEs, $\s$ is the spatial index, and $t$ denote the temporal index.
% To give a concrete example, the $u_i$, $i=1,\hdots,4$, could refer to velocity components (say $i=1,2,3$) and pressure ($i=4)$ in a fluid flow model. 
The PDEs can be fully nonlinear and parameterized in an arbitrary fashion (including the initial and boundary conditions); they are also assumed to be well-posed (\ie solutions always exist and are unique) for the range of values of $\x$ considered.

The quantity of interest is the function $u(\x,\s,t)$ in the given range of $\x$.
Direct approximation of this function is difficult due to the amount of samples we need to cover the response surface for such a high-dimensional space~\citep{higdon2008computer}.
Instead, we can record values at specified (fixed) spatial locations, $\s_i$, $i=1,\dots,d_s$, and temporal locations, $t_i$, $i=1,\dots,d_t$.
For different input parameters $\x_i\in \mathbb{R}^l$, the  outputs of the simulator are represented as vectors: $\y^{(F)}_i = \y^{(F)}(\x_i) = (u(\x_i,\s_1,t_1),...,u(\x_i,\s_{d_s},t_{d_t}))^T \in \mathbb{R}^d$, where $d=d_s\times d_t$. 
Here, we use the superscript ${(F)}$ to denote that the resulting vector is from an accurate, high-fidelity simulation.
%As is suggested in \citep{higdon2008computer},
The value at different spatial-temporal locations can be achieved easily through interpolation provided that the spatial-temporal fixed points are dense enough; interpolation in this case comes with ignorable extra computational effort~\citep{higdon2008computer}.
With the preceding process, the simulation is now treated as a mapping from $\mathbb{R}^l$ to $\mathbb{R}^d$, where $d$ is extremely large.
The goal of a data-driven surrogate is to approximate the mapping given training set $\mathcal{D} = \{\X, \Y^{(F)}\}$, where $\X = [\x_1,\ldots,\x_N]^T$ and $\Y^{(F)} = [\y^{(F)}_1,\ldots,\y^{(F)}_N]^T$.
%where $\y^{(F)}_i$ denotes the finest fidelity data that are very close to the ground truth value and the corresponding inputs $\x_i$ are referred to as {\/\it design inputs\/}. 
Provided that we have adequate number of samples to cover the response surface, we can approximate the mapping accurately.

As discussed in the introduction, we intend to avoid relying on only high-fidelity data. 
%In practice, getting accurate high fidelity data is computational expensive; it is impractical to get enough samples to cover the response surface of our interest.
The low-fidelity data can be cheaply obtained by reducing the fidelity setting (\eg the number of nodes of a discretization mesh and the order of basis functions of the finite element method) of a simulator.
In general, we can run a simulation at different fidelity settings to obtain a multi-fidelity dataset $\{\X^{(f)}, \Y^{(f)}\}_{f=1}^F$, where $\Y^{(f)}$ is a $N_f\times d$ matrix for observations at fidelity-$f$ with $\X^{(f)}$ being an $N_f\times l$ matrix for the corresponding inputs.
We use $f=F$ to denote the highest fidelity and $f=1$ the lowest.
%It is, however, practically easy to compromise the accuracy by ruining a simulator, given input $\x_i$ in a lower fidelity setting to collect cheaper but less accurate observation $\y_i^{(F-1)}$ and even cheaper observation $\y_i^{(F-2)}$.
%We denote the all fidelity data by 
Following the common setting for multi-fidelity data in~\citep{perdikaris2017nonlinear,cutajar2019deep}, we also require that the training inputs of fidelity $f$ is a subset of the previous fidelity $f-1$, .i.e, $\X^{(f)} \subset \X^{(f-1)}$. For convenience, 
% It is obvious that for $f\geq2$, $\X^{(f)} \subset \X^{(1)}$.
we introduce the index notation $\e$ to extract rows form a standard matrix such that $\X^{(f)} = \X_{\e_f,:}$, where $\e_f$ indicates the subset indexes for fidelity data $f$ and $\X$ contains all candidates.
Our goal of surrogate model becomes: given multi-fidelity data $\{\X^{(f)}, \Y^{(f)}\}_{f=1}^F$, how do we efficiently approximate the mapping between $\x$ and $\y^{(F)}$.


%It is assumed for now that a single output $\mbox{\textbf{\textit{y}}}$ (derived from a single scalar field $u({\textbf{\textit{x}}};{\pmb{\xi}})$) is the target for emulation. 
%
%From the preceding discussion, the simulator can be considered as a mapping $\pmb{\eta}:{\cal X}\rightarrow {\cal M}$ (assumed to be injective), where ${\cal M}\subset \mathbb{R}^d$ is the permissible output space (response surface) and ${\cal X} \subset \mathbb{R}^l$ is the permissible input space. That is, $\pmb{\eta}(\pmb{\xi})= \mbox{\textbf{\textit{y}}}=(u(\textbf{\textit{x}}^{(1)};\pmb{\xi}),\dots,u(\textbf{\textit{x}}^{(d)};\pmb{\xi}))^T$ for an arbitrary input $\pmb{\xi}$. 

%To infer outputs of the simulator at new inputs, Conti and O'Hagan~\cite{Conti2010} took the approach of placing a $d$-dimensional GP prior over $\pmb{\eta}$, indexed by $\pmb{\xi}$.  Effectively, the same assumption was made by Higdon {\/\em et al.\/}~\cite{Higdon} but in that case the outputs were a linear combination of PCA basis vectors with coefficients  treated as independent univariate GPs indexed by $\pmb{\xi}$. In this paper, a similar approach is adopted but rather than using PCA coefficients  we place GP priors over coefficients of a reduced-dimensional approximation of  points in ${\cal M}$, obtained by manifold learning methods. We assume that  ${\cal M}$ is a smooth manifold in $\mathbb{R}^d$. The high dimension $d$ of the output space  and the inability of linear dimensionality reduction methods such as PCA to capture complex response surfaces  is the motivation for our approach. 

\section{Model Formulation}
%problem definiteion --- deep gp (with introduction of sgp) --- lmc model --- deep lmc model 

\subsection{Univariate Gaussian Process}
\label{sec:sgp}
We first review the GP regression for learning a univariate function using a high-fidelity dataset $\Dcal = \{\X, \Y^{(F)}\}$.
The quantity of interest is assumed univariate, i.e., $d=1$. We use $y^{(F)}_i$ to distinguish a univariate observation from a multivariate one $\y^{(F)}_i$.
%where each $\x_i$ is a $l$ dimensional input vector, and $y^{(F)}_i$ the observed scalar output, we aim to learn a function $f: \mathbb{R}^p \rightarrow \mathbb{R}$. 
A GP assumes that the finite set of function values on $\X = [\x_1, \ldots, \x_N]^\top$, namely $\y^{(F)} = [y^{(F)}_1, \ldots, y^{(F)}_N]^\top$, follows a multivariate Gaussian distribution, 
$p(\y^{(F)} | \X) = \N(\y^{(F)} | \m, \K + \tau^{-1} \I)$.
Here $\m = [m(\x_1), \ldots, m(\x_n)]^\top$ is the mean function that is usually set to $\0$ after centering $\Y^{(F)}$, and 
$\tau$ is the inverse noise variance, which accounts for model inadequacies and numerical error~\citep{kennedy2001bayesian,rasmussen2003gaussian}.
$\K$ is the covariance matrix with elements $[\K]_{ij} = k(\x_i, \x_j)$, where $k(\x_i, \x_j)$ is a kernel function for the corresponding inputs.
Choosing the right kernel function for a specific application is nontrivial. 
When there is no prior knowledge to guide the choice, the automatic relevance deterrence (ARD) kernel \citep{rasmussen2003gaussian},
\begin{equation}
	k(\x_i, \x_j) = \theta_0 \exp\left(-(\x_i-\x_j) \diag(\theta_1,\ldots,\theta_l) (\x_i-\x_j)^T \right),
\end{equation}
is often utilized. The ARD kernel can freely capture the individual influence of each input parameter on the output results.
The hyperparameters $\{\tau,\theta_0, \ldots, \theta_l\}$ can be estimated by maximizing  the  marginal likelihood of the GP regression,
\begin{equation}
\label{eq:sgp likelihood}
\Lcal = \frac{1}{2} \ln|\K + \tau^{-1} \I| - \frac{1}{2}{\y^{(F)}}^T (\K+\tau^{-1} \I)^{-1} \y^{(F)} - \frac{N}{2} \ln(2\pi).
\end{equation}
The main computational cost is the inversion of $\K$, which is $\Ocal(N^3)$ and $\Ocal(N^2)$ for time and space complexity, respectively.
Given a new input $\x_*$, we can derive its posterior using a conditional Gaussian distribution,
\begin{equation}
\label{eq:sgp}
\begin{aligned}
 p\big(y^{(F)}_*|\x_*, \X,\y\big) &= \N\left(y^{(F)}_* | \mu(\x_*), v(\x_*)\right) \\
 \mu(\x_*) &= \k_{*}^\top (\K + \tau^{-1} \I)^{-1}\y^{(F)} \\
 v(\x_*) &= k(\x_*, \x_*) - \k_{*}^\top(\K + \tau^{-1}\I)^{-1}\k_{*},
\end{aligned}
\end{equation}
where, $\k_{*} = [k(\x_*, \x_1), \ldots, k(\x_*, \x_{N_F})]^\top$ is the vector of covariance between $\x_*$ and $\X$. 

%The inference of the GP regression is to estimate the covariance (or kernel) parameters (\eg $\{\theta_0, \ldots, \theta_l\}$ in the ARD  kernel) and the inverse noise variance $\tau$ that best explain the observed data $\Dcal$.
%We can optimize these hyperparameters by maximizing  the  marginal likelihood likelihood,
%\begin{equation}
%\label{eq:sgp likelihood}
%	\Lcal = \frac{1}{2} \ln|\K| - \frac{1}{2}\Y^T \K^{-1} \Y - \frac{N}{2} \ln(2\pi).
%\end{equation}
%The main computational cost is the inversion of $\K$, which takes $\Ocal(N^3)$ and $\Ocal(N^2)$ time and space complexity, respectively.

\subsection{Linear Model of Coregionalization}
In order to model the high-dimensional output correlations within limited computational resources, the linear model of coregionalization~\citep{matheron1982pour} assumes a separable decomposition structure,
%we borrow the classic multiple output Gaussian process framework------to decompose the $f$ fidelity high dimensional output,
%which assumes a linear low-rank structure for the high dimensional output as,
%The LMC represents the a multiple output as a linear combination of $R$ latent process,
\begin{equation} \label{eq:lmc}
\y^{(F)}(\x) = \sum_{r=1}^{R_f} \b^{(F)}_r z^{(F)}_r(\x) = \B^{(F)} \z^{(F)}(\x). 
\end{equation}
In this formulation, 
$\B^{(F)} = [\b^{(F)}_1,\dots,\b^{(F)}_{R_f}]$ is the collection of bases $\b^{(F)}_r \in \mathbb{R}^d$; $\z^{(F)}(\x) = [\z^{(F)}_1(\x),\dots,\z^{(F)}_{R_F}(\x)]^T$ is the collection of corresponding latent processes, \ie GPs.
%This is equivalent to define a matrix GP prior for the finite observations,
%\begin{equation}
%\vec(\Y^{(F)}) = \mathcal{N}(\0, \K_d \otimes \K+\tau^{-1} \I)
%\end{equation}
It is assumed that the latent processes are independent (i.e., $\cov( z^{(F)}_r(\x), z^{(F)}_{r'}(\x')) = 0$ for $r \neq r'$) and the bases are orthogonal (${\B^{(F)}}^T \B^{(F)}=\I$).
The LMC model essentially assumes several independent latent processes to fully characterize the data variability. 
The model has been shown particularly effective for the emulations of fields problems~\citep{higdon2008computer}.
%It is shown particularly efficient for the simulation field problems\citep{higdon2008computer}.
The formulation implicitly places the following GP prior:
\begin{equation}
\label{eq:lmc in sum}
\y^{(F)}(\x) = \mathcal{N}(\0, \sum_{r=1}^{R_F} b_r b_r^T k_r(\x, \x') ).
%= \mathcal{N}\left(\0, \sum_{r=1}^{R_F} \B_r k_r(\x, \x') \right).
\end{equation}
Given the high-fidelity observations $\{\X, \Y^{(F)}\}$, we can derive the posterior
\begin{equation}
\label{eq:lmc post}
\begin{aligned}
p\big(\y^{(F)}_*|\x_*, \X,\y\big) &= \N\left(\y^{(F)}_* | \bmu(\x_*), \v(\x_*)\right) \\
\bmu(\x_*) &= \sum_{r=1}^{R_F} \b_r^{(f)} \k_{r*}^\top (\K_r + \tau_r^{-1} \I)^{-1}\Y^{(F)}\b_r^{(f)} \\
\v(\x_*) &= \sum_{r=1}^{R_F} \b_r^{(f)} \left(k_r(\x_*, \x_*) - \k_{r*}^\top(\K_r + \tau_r^{-1}\I)^{-1}\k_{r*}\right) {\b_r^{(f)}}^T,
\end{aligned}
\end{equation}
where $\k_{r*} = [k_r(\x_*, \x_1), \ldots, k_r(\x_*, \x_{N_F})]^\top$ is the vector of covariance between $\x_*$ and $\X$. 
We can see that flexibility of the posterior of $\y^{(F)}_*$ is heavily determined by the size of $\K_r$, which is the number of high-fidelity samples $N_f$. 

%Lemma:
%The formulation implicitly place the following GP prior for the observations,
%\begin{equation}
%\cov (\y(\x), \y(\x')) = \sum_r \b^{(f)}_r \cov(z^{(f)}_r(\x)) {\b^{(f)}_r}^T
%= \sum_r \b^{(f)}_r {\b^{(f)}_r}^T k_r(\x, \x')
%\end{equation}
%Assuming $\{\B^{(f)}\}_{f=1}^F$ is known, we can substitute Eq.~\eqref{eq:lmc} into Eq.~\eqref{eq:deep gp} to derive the deep latent process for the LMC model,
\subsection{Deep Gaussian Process Auto-regression}
%\subsection{Deep Coregionalization}
Before we move to our model, we make a brief review of deep GP auto-regression, which is used later to derive our model.
Let us consider the multi-fidelity, univariate data,
\ie $\{\X^{(f)},\Y^{(f)}\}_{f=1}^F$ where $\Y^{(f)} = [y^{(f)}_1,\ldots,y^{(f)}_{N_f}]^T $ is a collection of samples at fidelity $f$.
%First, let consider the traditional GP for multi-fidelity data where the quantity of interest is a univariate, i.e., $d=1$ for our problem. We use $y$ to distinct the univariate observations from a multivariate one $\y$.
The general auto-regressive formulation for multi-fidelity data is
% data put forward by \citep{perdikaris2017nonlinear} is
\begin{equation}
y^{(f)}(\x) = g^{(f)}\left(y^{(f-1)}(\x)\right) + \epsilon^{(f)},
\end{equation}
where $g^{(f)}(y^{(f-1)}(\x))$ is an arbitrary function that maps the low-fidelity results to the high-fidelity ones and $\epsilon^{(f)}$ captures the model inadequacies and numerical errors.
If we assume a simple linear form for the mapping, i.e.,  $g^{(f)}(y^{(f-1)}(\x)) = c \cdot y^{(f-1)}(\x)$, we recover the classic auto-regressive model~\citep{kennedy2000predicting}.
This method is further improved by \citet{le2013multi}, who used a deterministic parametric form of $g^{(f)}$ and an efficient numerical scheme to reduce the computational cost. 
Despite successfully dealing with some demonstrated problems, 
this parametric approach does not generalize well due to the difficulty of model selection and the demand for large training datasets~\citep{perdikaris2017nonlinear}.
To resolve this issue, a Bayesian non-parametric treatment can be implemented by placing a GP prior over the function $g^{(f)}$.
This is also known as the \textit{deep GP}~\citep{damianou2013deep}.
Although being capable of modeling complex problem, deep GP is infamous for its intractability. It requires computationally expensive variational approximation for model training and thus quickly becomes infeasible for multi-fidelity simulation problems.
\citet{perdikaris2017nonlinear} put forward a GP-based nonlinear autoregressive scheme with an additive structure,
\begin{equation} \label{eq:deep gp}
y^{(f)}(\x) = g^{(f)}\left(\x, y_*^{(f-1)}(\x)\right),
\end{equation}
where the error term is absorbed into $\g^{(f)}(\x)$, and
$\y_*^{(f-1)}(\x)$ is the posterior for $\x$ at fidelity $(f-1)$.
 This formulation specifies that $\y^{(f)}(\x)$ is a GP given the previous fidelity observations and the model inputs.
%which is effective for the multi-fidelity problem.
To better reflect the autoregressive nature, \citet{perdikaris2017nonlinear} suggested a covariance function that decomposes as
\begin{equation}
\label{eq:deep gp kernel}
\begin{aligned}
&k^{(f)}\left([\x, y_*^{(f-1)}(\x)], [\x',y_*^{(f-1)}(\x')]\right)\\ &=  k_x^{(f)}(\x, \x'; \btheta_{fx} ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x), y_*^{(f-1)}(\x'); \btheta_{fy} ),
%+k_{\delta}^{(f)}(\x, \x'; \btheta_{f\delta}),
\end{aligned}
\end{equation}
where $k_x^{(f)}$ and $k_y^{(f)}$ are valid covariance functions with $\{\btheta_{f_x}, \btheta_{f_y}\}$ denoting the corresponding hyperparameters.
%is also implemented.
These hyperparameters could be learned via maximum-likelihood estimation as in Eq.~\eqref{eq:sgp likelihood} using input data $\{\X^{(f)}, \Y^{(f-1)}\}$ and output data $\Y^{(f)}$.
Thus, unlike the standard deep GP~\citep{damianou2013deep}, this autoregressive model does not have the intractable issues for estimating the unknown latent variables and hyperparameters.
%using available design input and related fidelity data. 
This method requires estimation of $(l+3)$ hyperparameters with an ARD kernel for each fidelity model.

\subsection{Deep Coregionalization}
Despite being much more efficient than the full deep GP with variational inference, the GP autoregressive model does not naturally extend to multivariate cases, especially to those of very high dimension. 
%First, the correlation function will need to encode the output correlation using a more complicated kernel function such as $k^{(f)}\left(\x, \x', \y(\x), \y(\x'), i,j \right)$, where $i$ and $j$ denotes the $i-th$ and $j-th$ output.
First, it considers the outputs in each layer as independent (given the inputs),and it is unclear how to model the strong output correlations, which is crucial for learning with a small set of training examples. 
%While we can extend Equation\eqref{eq:deep gp} to a standard deep GP that samples multiple functions in each layer, it feeds all the outputs into the next layer and hence is not scalable to a large number of outputs, say, millions. 
Second, when using an anisotropic kernel such as the ARD, the deep kernel function $k_y^{(f)}$ in Eq.~\eqref{eq:deep gp} requires $d$ hyperparameters to be optimized, which is practically impossible for our problem where $d$ can scale up to 1 million.

\cmt{
\subsection{Deep Linear Model of Coregionalization}
In order to model the high dimensional output correlations within limited computational resources, we borrow the classic multiple output Gaussian process framework---Linear Model of Coregionalization (LMC)~\citep{matheron1982pour}---to decompose the $f$ fidelity high dimensional output,
%which assumes a linear low-rank structure for the high dimensional output as,
%The LMC represents the a multiple output as a linear combination of $R$ latent process,
\begin{equation} \label{eq:lmc}
\y^{(f)}(\x) = \sum_{r=1}^{R_f} \b^{(f)}_r z^{(f)}_r(\x) = \B^{(f)} \z^{(f)}(\x). 
\end{equation}
In this formulation, 
$\B^{(f)} = [\b^{(f)}_1,\dots,\b^{(f)}_{R_f}]$ is the collection of bases $\b^{(f)}_r \in \mathbb{R}^d$; $\z^{(f)}(\x) = [\z^{(f)}_1(\x),\dots,\z^{(f)}_{R_f}(\x)]^T$ is the collection of corresponding latent processes.
It is assumed that the latent processes are independent, i.e., $\cov( z^{(f)}_r(\x), z^{(f)}_{r'}(\x')) = 0$ for $r \neq r'$ and the bases are orthogonal.
The LMC model essentially assumes several independent latent processes to fully characterize the data variability. It is shown particularly efficient for the simulation-type problems\citep{higdon2008computer,zhe2019scalable}.
}

\cmt{
To model the output correlations, let's modify Eq.~\eqref{eq:deep gp kernel} using a general separable structure as
\begin{equation}
\label{eq:deep gp kernel2}
\begin{aligned}
&\cov\left(y_{i}^{(f)}(\x),y_{j}^{(f)}(\x') \right)  =
 k^{(f)}_d(i,j)  \cdot k^{(f)}\left([\x, y_*^{(f-1)}(\x)], [\x',y_*^{(f-1)}(\x')]\right) + \tau^{-1} \\
&=  k^{(f)}_d(i,j)  \cdot k_x^{(f)}(\x, \x' ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x), y_*^{(f-1)}(\x')) + \tau^{-1},
\end{aligned}
\end{equation}
%We can equivalently derive the covariance matrix between high-dimensional outputs,
which give rise to the covariance matrix between high-dimensional outputs,
\begin{equation}
%\label{eq:deep gp kernel2}
\begin{aligned}
\cov\left(\y^{(f)}(\x),\y^{(f)}(\x') \right)
=  \K^{(f)}_d   \cdot k_x^{(f)}(\x, \x' ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x) y_*^{(f-1)}(\x')) + \tau^{-1} 
\end{aligned}
\end{equation}
We immediately recognize this is a simplified case of Eq.~\eqref{eq:lmc in sum}, where $\b_r = \v^{(f)}_r \sqrt{\lambda^{(f)}_r}$ and $k_r(\x,\x') =  k_x^{(f)}(\x, \x' ) \cdot k_y^{(f)}(y_*^{(f-1)}(\x) y_*^{(f-1)}(\x'))$. $\v_r$ and${\lambda_r}$ are the eigenvector and eigenvalue of $\K^{(f)}_d$ here.
Thus, we can write $\y^{(f)}(\x)= \B^{(f)}z(\x) $ as in Eq.\eqref{eq:lmc}.
Similarly, 



With some linear algebra (details are supplied in Appendix XX), we can show that the separable structure is equivalent to specify that 
\begin{equation}
\y^{(f)}(\x) = \v k_y^{(f)}(y_*^{(f-1)}(\x), y_*^{(f-1)}(\x')),
\end{equation}

}
LMC has shown to be general and applicable for decomposing fine-fidelity spatial-temporal fields $\y^{(f)}(\x)$ ~\citep{higdon2008computer}. Thus, without loss of generality, we can assume that 
%The LMC model essentially assumes several independent latent processes to fully characterize the data variability. It is shown particularly efficient for the simulation-type problems\citep{higdon2008computer,zhe2019scalable}.
all high-dimensional outputs from different fidelities also admit the LMC decomposition, \ie $\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x)$. Substitute the formulation into Eq.~\eqref{eq:deep gp}, we have
%Assuming $\{\B^{(f)}\}_{f=1}^F$ is known, we can substitute Eq.~\eqref{eq:lmc} into Eq.~\eqref{eq:deep gp} to derive the deep latent process for the LMC model,
\begin{equation}
\begin{aligned}
\B^{(f)} \z^{(f)}(\x) & = \g^{(f)}\left(\x, \B^{(f-1)} \z_*^{(f-1)}(\x)\right)\\
\z^{(f)}(\x) & = {\B^{(f)}}^T \g^{(f)}\left(\x, \B^{(f-1)} \z_*^{(f-1)}(\x)\right)\\
\z^{(f)}(\x) & = \hat{\g}^{(f)}\left(\x,\z_*^{(f-1)}(\x)\right),\\
\end{aligned}
\label{eq:deep lmc1}
\end{equation}
where $\hat{\g}^{(f)}$ is the composite function absorbing $\B^{(f)}$ and $\B^{(f-1)}$ into the multivariate mapping $\g^{(f)}$.
%Generally, $\hat{\g}^{(f)}$ is not necessary a multivariate GP given that $\g^{(f)}$ is a multivariate GP. Nevertheless, we can show that for a multivariate GP with the commonly assumed separable structure, $\hat{\g}^{(f)}$ is a Gaussian 
\begin{theorem}
\label{THEOREM1}
If the high-dimensional GP autoregression $\g^{(f)}(\x,\y_*^{(f-1)}(\x))$ admits an LMC formulation, $\hat{\g}_r^{(f)}$ must exist and can be decomposed into several independent univariate GPs, $\{\hat{\g}_r^{(f)}(\x,\z_*^{(f-1)}(\x))\}_{r=1}^{R_f}$.
\end{theorem}
We provide the proof in Appendix \ref{ap:proof t1}.
With this conclusion, we can see that the high-fidelity field depends only on the latent process of its previous fidelity and the inputs once the bases are found. The output correlations are captured independently for each fidelity, whereas the fidelity correlations are propagated through independent univariate GPs. We thus call the model \textit{deep coregionalization}.
The joint likelihood given the multi-fidelity data is
\begin{equation} 
\label{eq:dc likelihood}
\Lcal \propto \sum_{f=1}^{F}  \sum_{r=1}^{R_f} \frac{1}{2}  \ln|\bSigma_{fr}| - \frac{1}{2}\tr\left({\z^{(f)}_r}^T \bSigma_{fr}^{-1} \z^{(f)}_r \right),
% - \frac{R_f N_f}{2} \ln(2\pi),
\end{equation}
%
where $\z^{(f)}_r = \Y^{(f)}\b_r^{(f)}$ is the projection of $\Y^{(f)}$ onto base $\b_r^{(f)}$, $\bSigma_{fr} = \K_{fr} + \tau^{-1} \I$ is the covariance matrix with the noise term for r-th latent process of f-fidelity observations, 
%$\K_{fr}$ is as defined in Eq. \ref{eq:deep gp kernel}.
and $[\K_{fr}]_{ij} = k_{fr}\left(\x_i,\z^{(f-1)}(\x_i),\x_j,\z^{(f-1)}(\x_j) \right)$ is the covariance matrix for the latent process $\hat{\g}_r^{(f)}(\x,\z_*^{(f-1)}(\x))$ based on its own kernel function $k_{fr}$ and inputs $\X^{(f)}$ and $\Z^{(f-1)}_{\e_f,:}$
%------------
% use the low-fidelity latent process to improve the predictions of high-fidelity latent process. 
%In cases where the original high-dimensional GP $\g^{(f)}$ does not have a separable structure, without loss of generality, we can still place a Gaussian prior over $\hat{\g}^{(f)}$ as an non-parametric Bayesian regression.

% assume a multivariate GP as in the univariate deep GP and place a Gaussian prior over 
%
%The only difference form the univariate case is that this GP is multivariate. However, 
%\subsection{Model Training}
%Model training, \ie maximizing the likelihood function \ref{eq:dc likelihood}, is non-trivial.
% First, we do not 
% each basis contains 
 
%Since the LMC requires the latent process to be independent from each other, Eq.~\eqref{eq:deep lmc1} further decomposes as
%\begin{equation}
%z_r^{(f)}(\x) = \hat{g}_r^{(f)}\left(\x,\z_*^{(f-1)}(\x)\right),
%\end{equation}
%where each $\hat{g}_r^{(f)}$ is an independent GP and could be modeled separately using the univeriate GP model introduced in section~\ref{sec:sgp}. 
%Since we will have limited high-fidelity data, we adopt a conditional independent approach, \ie the latent processes are independent given the same hyperparameters. The marginal likelihood of the conditional independent latent process at fidelity $f$ is
%\begin{equation}
%\label{eq:cigp likelihood}
%\Lcal_f = \frac{R_f}{2} \ln|\K_f| - \tr\left(\frac{R_f}{2}{\Z^{(f)}}^T \K_f^{-1} \Z^{(f)}\right) - \frac{R_f N_f}{2} \ln(2\pi),
%\end{equation}
%where $[\K_f]_{ij} = k_f\left(\x_i,\z_*^{(f-1)}(\x_i),\x_j,\z_*^{(f-1)}(\x_j) \right)$ is the covariance matrix and $\Z^{(f)}=[\z(\x_1)^T,\ldots,\z(\x_{N_f})^T]^T$ is the collection of latent process coefficients.

%The conditional independent assumption reduce the hyperparameters from $R_f(R_{f-1}+3)$ to $R_{f-1}+3$ and computation complexity from $\Ocal(R_f N_f^3)$ to $\Ocal(N_f^3)$ compared to the fully independent approach.


%\begin{lemma}
%\label{lemma1}
%A LMC model assumes a multivariate Gaussian prior:
%\begin{equation*}
%\begin{aligned}
% \y^{(f)}(\x) &= \mathcal{N}(\0, \B^{(f)} \K^{(f)}(\x,\x') {\B^{(f)}}^T )\\
%\K^{(f)}(\x,\x') &= \diag\left(k^{(f)}_1(\x,\x'),\dots,k^{(f)}_R(\x,\x') \right).
%\end{aligned}
%\end{equation*}
%\end{lemma}
%We leave the proof in the Appendix. This property allow us to substitute the LMC in the GP autoregressive model without adding more assumption and to derive the following:
%\begin{lemma}
%\label{lemma2}
%	With the LMC representation, the deep kernel always has a equivalent compact kernel function based on previous latent process posterior,
%	\[	k^{(f)}\left(\x, \x', \y_*^{(f-1)}(\x), \y_*^{(f-1)}(\x')\right) = \hat{k}^{(f)}\left(\x, \x', \z_*^{(f-1)}(\x), \z_*^{(f-1)}(\x)\right). \]
%\end{lemma}
%
%With lemma \ref{lemma1} and \ref{lemma2}, we now derive a low-rank equivalent GP autoregressive model: 
%\begin{prop}
%	If each fidelity date admits a LMC representation, there exist a low-rank independent deep structure that fully capture the information of data and uncertainty,
%	\[
%	z_r^{(f)}(\x) = \widehat{g}_r^{(f)}(\x, \z_*^{(f-1)}(\x)).
%	\]
%\end{prop}
%Now the high dimensional deep GP is disentangled into multiple low dimensional univariate GPs that are free from massive hyperparameters and complex multivariate model.

\subsection{Residual Principal Component Analysis}
The challenge for \ours is the optimization of the bases $\B^{(f)}$ and the low-rank $R_f$ for each fidelity.
If we set $R_f=1$ for each fidelity data, we recover the \textit{intrinsic coregionalization model} (ICM)~\citep{goovaerts1997geostatistics} where an efficient Kronecker structure could be utilized to speed up the computation. However, the model capacity can be quite limited due to the oversimplified latent process. A larger $R_f$ enables us to model outputs with different characteristics~\citep{alvarez2012kernels} with the cost of more hyperparameters to infer.
The output correlation can be indirectly modeled using a full-rank or low-rank Cholesky decomposition to allow flexible output correlations~\citep{bonilla2008multi}.
The number of parameters to infer for the aforementioned methods is proportional to $d \times R_f$, resulting into a impractical approach for high-dimensional outputs.  
%They are thus not suitable our application considering the large $d$.
% and the scarce high fidelity data. 
%These aforementioned methods all require joint learning $d\times R$ hyperprameter to encode the spatial correlation. This can be problematic for our application considering the large $d$ and the scarce high fidelity data.
Since the simulation outputs are always complete and can be efficiently represented via principal components~\citep{ramsey1997functional},
\citet{higdon2008computer} suggested using the principal components as the bases. 
More specifically, after standardizing the data, singular value decomposition (SVD) is applied to $\Y^{(f)}$, and the first $R_f$ left singular vectors are then used as the bases $\B^{(f)}$.
%for $\Y^{(f)}$, we can first standardize the result in a $N_f \times d$ matrix $\widetilde{\Y}^{(f)}$ and obtain the bases matrix $\B$ by using the first $R$ principal components of $\widetilde{\Y}^{(f)}$.
Another benefit of this approach is a heuristic method to choose the number of bases by choosing $R_f$ such that at least $90\%$ of the variance of the output is covered by the bases. 
It is reported that the components that explain minor trend of the variation do not add to the predictive ability of the GP model~\citep{higdon2008computer}.

This approach works well for many single-fidelity applications~\citep{higdon2008computer,zhe2019scalable}, but a direct implementation to our model here is inappropriate.
%First, for high fidelity data, $\Y^{(f)}$ where $f$ is large, the data is scarce.
First, the principal components (the bases) are essentially based on the empirical covariance matrix given data $\Y^{(f)}$. 
Since we can afford to have only limited number of high-fidelity samples, the empirical covariance matrix is a very rough approximation to the real one, and the resulting principal components are consequently inaccurate.
Second, even provided that we are always given enough samples to explore the output correlation at each fidelity, direct implementation of \citet{higdon2008computer} is of low efficiency.
According to our experiments, when directly implementing SVD, the dominant components and their corresponding coefficients for each fidelity are always similar.
The similarity implies that a using a complicated nonlinear model, \eg GP, to propagate such a simple correlation in a deep structure is of low efficiency and may lead to inferior model accuracy.
%The similarity means propagating these coefficients in the deep latent process is of low efficiency. 
Instead, we can limit the information passing down the model and only model the updated (added) information.
%To take the advantage of such nature, rather than applying \citet{higdon2008computer} to each fidelity data, we apply it to the residual the information. 
%To avoid this issues, we introduce a residual structure. 
Specifically, we specify
\begin{equation}
\begin{cases}
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) \;\; &\mathrm{for} \; f = 1 \\
\y^{(f)}(\x) = \B^{(f)} \z^{(f)}(\x) + \y^{(f-1)}(\x)  \;\; &\mathrm{for} \; f \geq 2. \\
\end{cases}
\end{equation}
In this formulation, each fidelity layer learns the residual (additional) information compared with the previous fidelity layer rather than the whole output information, and thus we call this a \textit{residual deep structure} similar to the work of \citet{he2016deep}.
%We call this formulation \textit{residual principal component analysis} since that for each fidelity data, we only need to 
%This formulation means that each fidelity model only need to learn the additional information compared with the previous fidelity model. 
%The lower fidelity models provide the low frequency signals while the higher fidelity models offer detailed information for the system.
Except for efficiency, another advantages of this approach is that the predictive posterior for high-fidelity results naturally decompose into an additive structure.
The additive structure can help us identify the main sources of uncertainty and adjust our model at each fidelity accordingly to reduce model uncertainty and improve model accuracy.
%
%An other benefit of this formulation is that, unlike traditional deep GPs, where the predictive uncertainty is propagated and accumulating, our our method admit a additive uncertainty structure where the uncertainty for each 

Inspired by the practical approach of \citep{higdon2008computer} to extract the bases, we introduce the \textit{residual principal component analysis} (ResPCA) for our model. 
The method is a modification of PCA applied to the residual information instead of the original data. We use SVD, which is more numerical stable than direct eigendecomposition on the empirical covariance matrix, to extract the eigenvectors. The detailed steps of this method are presented in Algorithm~\ref{algo:rpca}.
%\begin{equation}
%\B^{(f)} = PCA(\Y^{(f)} - \Y^{(f-1)}) = \cov[\y^{(f)}(\x) - \y^{(f-1)}(\x)]
%\end{equation}
%\begin{equation}
%\var[\y^{(f)}(\x) - \y^{(f-1)}(\x)] = \EE[\y^{(f)}(\x) - \y^{(f-1)}(\x) -]
%\end{equation}
\begin{algorithm}[h]
	\caption{ResPCA}
	\label{algo:rpca}
	\begin{algorithmic}[1]
		\Require
		multi-fidelity multivariate data $\{\X^{(f)},\Y^{(f)} \}_{f=1}^F$ and index $\{\e_{f}\}_{f=1}^F$;
		\Ensure
		Residual bases $\{\B^{(f)}\}_{f=1}^F$;
		Residual coefficients $\{\Z^{(f)}\}_{f=1}^F$;
		\State $\B^{(1)} = \mathrm{SVD}({\Y}^{(1)})$; \; $\Z^{(1)} = {\Y}^{(1)} {\B^{(1)}}^T$
		\For{each $ f \in [2,F]$}
		\State Achieve residual information $\widetilde{\Y}^{(f)} = \Y^{(f)} - \Y^{(f-1)}_{\e_{f-1},:} $
%		\State Standardize  $\widetilde{\Y}$
		\State Achieve residual base $\B^{(f)} = \mathrm{SVD}(\widetilde{\Y}^{(f)})$
		\State Achieve residual coefficient $\Z^{(f)} =  {\B^{(f)}}^T \widetilde{\Y}^{(f)}$
		\EndFor
		\label{code:recentEnd}
	\end{algorithmic}
\end{algorithm}
%With the bases derived from ResPCA, 
We can now substitute the projections of residual information $\Z^{(f)}$ into Eq.~\ref{eq:dc likelihood} for model training.

\subsection{Prediction and Uncertainty Propagation}
Due to the intractability of a deep GP structure, except for the latent posterior $\z^{(1)}(\x)$ corresponding to the lowest fidelity $\y^{(1)}(\x)$, the predictive latent posterior for each fidelity is
\begin{equation}
\label{eq:dgp posterior}
\z_*^{(f)}(\x) = \int \g^{(f)}\left(\x, \z_*^{(f-1)}(\x) \right) p\left(\z_*^{(f-1)}(\x)\right) d \z_*^{(f-1)}(\x).
\end{equation}
%for $\space f=2,\ldots,F$.
This integral is intractable and the posterior is no longer a Gaussian, but we can approximate it numerically using sampling-based methods. We can further reduce the complexity due to the independent assumption of the LMC; Eq.~\eqref{eq:dgp posterior} naturally decomposes as
\begin{equation}
\label{eq:dgp posterior decomp}
\z_{*}^{(f)}(\x) =  \prod_{k=1}^{R_f} \int g_k^{(f)}\left(\x, \z_*^{(f-1)}(\x) \right) \prod_{r=1}^{R_{f-1}} p(z_{*r}^{(f-1)}(\x)) d z_{*r}^{(f-1)}(\x).
\end{equation}
We can now easily implement a Monte Carlo sampling method to calculate the latent process posteriors. Another way to solve the intractable integral is to apply a Gaussian approximation of each latent posterior as in \citet{perdikaris2017nonlinear} and \citet{girard2003gaussian}.
Once we obtain the approximated posterior, the first two order statistic admits a tractable solution due to the summation structure.
%For clarity, we organize all the bases and latent variable together, \ie 
%$\mathcal{B} = [\B^{(1)},\ldots,\B^{(F)}]$ 
%and $\mathcal{Z}(x) = [\z^{(1)}(\x),\ldots,\z^{(F)}(\x)]$.
%We can show that the first two statistical moments have a close form solution as,
%\begin{lemma}
%\label{LEMMA1}
Given the posterior of the latent processes $\z^{(f)}(\x)$ and the bases $\B^{(f)}$, the mean and variance of the finest fidelity field $\y^{(F)}(\x)$ can be calculated as
\begin{equation}
\begin{aligned}
\EE[\y^{(F)}(\x)] &= \sum_{f=1}^F \B^{(f)}\EE[\z_*^{(f)}(\x)],\\
\var[\y^{(F)}(\x)] &= 
%\B^{(1)}\var[\z^{(1)}(\x)]{\B^{(1)}}^T \\
\sum_{f=1}^F \left( \B^{(f)}\var[\z_*^{(f)}(\x)]{\B^{(f)}}^T \right)\\
&- 2 \sum_{f\neq f'} \left(\B^{(f)}\cov[\z_*^{(f)}(\x),\z_*^{(f')}(\x)]{\B^{(f')}}^T \right),
\end{aligned}
\label{eq:y post}
\end{equation}
%\end{lemma}
%Once we obtain the empirical posterior, we can calculate the mean prediction as,
%\begin{equation}
%\label{eq:dgp fmean}
%\EE[\y^{(F)}(\x)] = \sum_{f=1}^F \B^{(f)}\EE[\z^{(f)}(\x)].
%\end{equation}
%Since the latent posteriors are unknown distribution, the predictive variance is also intractable. However, we if we use a sampling based method, we can calculate the predictive posterior for the highest fidelity as,
%\begin{equation}
%\begin{aligned}
%\label{eq:dgp fvar}
% \var[\y^{(F)}(\x)] &= 
%%\B^{(1)}\var[\z^{(1)}(\x)]{\B^{(1)}}^T \\
% \sum_{f=1}^F \left( \B^{(f)}\var[\z^{(f)}(\x)]{\B^{(f)}}^T \right)\\
% &- 2 \sum_{f=2}^F \left(\B^{(f)}\cov[\z^{(f)}(\x),\z^{(f-1)}(\x)]{\B^{(f-1)}}^T \right)
%\end{aligned}
%\end{equation}
where $\var[\z^{(f)}(\x)]$ is the diagonal covariance matrix of the fidelity-$f$ latent posterior, and $\cov[\z^{(f)}(\x),\z^{(f')}(\x)$ is the covariance matrix of $\z^{(f)}(\x)$ and $\z^{(f')}(\x)$. This covariance matrix does not have an analytical form and 
can be calculated empirically using sampling methods. 
%We leave the proof of this result in the Appendix.
%with the samples we get in the sampling process.
%\textbf{we leave the proof of the result in the appendix.}
 
%\begin{corol}
%	Given 1st and 2nd order moment of $\z_*^{(f)}(\x_*)$,
%	% i.e., $\EE(\z_*^{(f)}(\x_*)) = \pmb\mu$ and $\cov(\z_*^{(f)}(\x_*)) = \bSigma^{(f)}$, 
%	the 1st and 2nd order moment of the field prediction has a close form as,
%	\begin{equation*}
%	\begin{aligned}
%		\EE(\y_*^{(F)}(\x_*)) &= \sum_{f=1}^F \B^{(f)}\EE(\z_*^{(f)}(\x_*)); \;\;\;\;\\
%		 \var(\y_*^{(F)}(\x_*)) &= \B^{(f)}\EE(\z_*^{(f)}(\x_*)) {\B^{(f)}}^T
%	\end{aligned}
%	\end{equation*}
%\end{corol}
%Further more, if $\z_*^{(f)}$ could be approximate using a multivariate Gaussian distribution $\z_*^{(f)}(\x_*)  \sim \N\left(\pmb\mu^{(f)}, \bSigma^{(f)} \right)$, then the output field $\y_*^{(f)}(\x_*) \sim \N\left(\B^{(f)}\pmb\mu^{(f)}, \B^{(f)}\bSigma^{(f)} {\B^{(f)}}^T \right)$ is also a multivariate Gaussian.

\subsection{Implementation and Model Complexity}
Before we describe our experiments, we review our model and the its implementation details for the emulation of spatial-temporal fields.
1). To build a surrogate model, We need to firstly collect different fidelity data from a simulator at design inputs $\X$. To better explore the response surface, we use a Sobol sequence~\citep{sobol1976uniformly} to generate the design points. For fidelity-$f$, we choose the first $N_f$ design points of $\X$ to generate the corresponding outputs $\Y^{(f)}$. The computational cost at this stage depends on the simulator and the fidelity setting.
2). We then apply Algorithm~\ref{algo:rpca} to get the residual bases $\{\B^{(f)}\}_{f=1}^F$ and corresponding projections $\{\Z^{(f)}\}_{f=1}^F$. The computational cost for fidelity-$f$ data is $\Ocal(\min(N_f^2 d,N_f d^2) )$ using SVD. For the choice of low-rank $R_f$, we can set a variance ratio as in \citet{higdon2008computer}. Specifically, the minimum number of bases to capture the variance ratio (calculated by the eigenvalues of the covariance matrix) is used.
%to decide the minimum number of base to capture
%In this work, we use a single low-rank for all fidelities, \ie $R=R_1=\ldots=R_F$.
%When $R$ is a integer, it indicates the actual number of base each fidelity use; when $R$ is a decimal fraction, it indicates the minimum number of base to capture the ratio variance for each fidelity is used by the model.
3). We maximize the joint likelihood function of Eq.~\eqref{eq:dc likelihood} w.r.t. the hyperparameters using gradient-based optimization method, \eg L-BFGS-B. 
This optimization consists of $\sum_{f=2}^{F}(R_f(R_{f-1}+3))$ hyperparameters and the computational complexity is $\Ocal(R_f N_f^3)$ per iteration.
In cases where we have very limited training data, we can instead place a conditional independent assumption~\citep{Lawrence06GPLVM} for $\hat{g}^{(f)}_r(\x,\z^{(f-1)}_*(\x))$, which reduces the hyperparameters to $\sum_{f=2}^{F} (R_{f-1}+3)$ and complexity $\Ocal(N_f^3)$ compared to the fully independent approach.
%The conditional independent assumption reduce the hyperparameters from $R_f(R_{f-1}+3)$ to $R_{f-1}+3$ and computation complexity from $\Ocal(R_f N_f^3)$ to $\Ocal(N_f^3)$ .
%For each pair of $\{ [\Z^{(f)},\Z^{(f-1)}_{e_f}],\X_{e_f})\}$, train $R_f$ independent GPs by maximizing the marginal log-likelihood of Eq.~\eqref{eq:sgp likelihood} when using fully independent GPs or Eq.~\eqref{eq:cigp likelihood} when using the conditional independent approach.
% The computational complexity, is $\Ocal(N_f^3 R_f)$ and $\Ocal(N_f^3)$, respectively for the two methods. 
%In this work, we use a L-BFGS-B for the optimization. 
%Though complete independent training can improve model flexibility, we found that conditional independent training, i.e., sharing the hyperparameter $\btheta^{(f)}$ for the independent latent GP produce more stable results with very little loss of model accuracy. With the conditional independent assumption, the complexity of each GP is $\Ocal(N_f^3)$. 
For large numbers of observations, sparse GPs~\citep{snelson2005sparse} can be placed on the latent process to reduce the computational cost.
4). Given a new $\x_*$, we calculate each latent posterior using Eq.~\eqref{eq:dgp posterior} and then compute the mean and variance of the highest fidelity outputs using Eq.~\eqref{eq:y post}.

%For high dimensional latent process, we can also apply a Gaussian approximation of all the residual posterior which yields closed form posterior\citep{perdikaris2017nonlinear,girard2003gaussian}. The first two moment of the field outputs can be derived using equation\eqref{label} once given the first two moment of the latent posterior.

%The simplest way is to specified $B$
%Implementation using PCA.
%Implementation of LMC can be done based on different way on defining the bases.
%For our application where the $d$ is very large, learning the bases jointly can be very difficult. Instead, we can use the PCA base from the data to construct the bases\citep{higdon2008computer}. 







==> relative_v1.tex <==
\section{Relative Work}
As a non-parametric method that can also quantify model uncertainty, 
Gaussian process (GP) is frequently used as the main data-driven surrogate model~\citep{santner2003design,Kennedy2006,Rougier2009,Tagade2013,Lee2013}.
Unfortunately, the GP doest not naturally extended to multiple outputs, especially those of very large dimension such as spatial-temporal fields.  
It might seem straightforward to simply treat the output indexes (indicating the field value at a particular location in the spatial-temporal domain for instance) as additional input parameters~\citep{kennedy2001bayesian}.
This approach is infeasible for high dimensional outputs since the computational complexity for a general GP is $\mathcal{O}(N^3d^3)$, where $N$ is the number of training sample and $d$ is the output dimensionality~\citep{McFarland2008}.
If we can assume a separable structure between the input covariance and the output covariance, the high computational issues could be circumvented efficiently.
Such a relaxation gives rise to the linear model of coregionalization (LMC)~\citep{matheron1982pour, goulard1992linear},  the classical framework for multi-output regression.
LMC linearly combines some bases with latent processes to predict the high dimensional output.
Many modern multi-output GP models can be considered special instances or variants of LMC~\citep{Konomi2014,Fricker2013,Rougier2008,zhe2019scalable}.
\citet{Conti2010} proposed a simplified LMC model, known as intrinsic coregionalization model (ICM)~\citep{Wackernagel}, which assumes a single latent process with a correlation matrix governing output correlations.
To relax the limitation of ICM, \citet{higdon2008computer} found a set of bases from Singular Value Decomposition(SVD) on the training outputs to encode the complicated spatial-temporal correlations for PDE simulation problems.
This approach is further extended by using nonlinear dimension reduction, such as Kernel PCA~\citep{xing2016manifold} and Isomap~\citep{xing2015reduced}.
Once the bases are identified and fixed, we only need to learn a small number of latent process using ordinary univariate GPs~\citep{Rasmussen06GP}. 
Hence, LMC can easily scale up to a large number of outputs.
Recent development of GP further introduces latent coordinate features to improve the flexibility of modeling complex output correlations~\citep{zhe2019scalable}. 

The main drawback of LMC is the separable assumption, which can be resolved by \textit{process convolution}~\citep{higdon2002space, boyle2005dependent,teh2005semiparametric, bonilla2008multi}.
The key idea is to derive high dimension outputs based on convolution between a smoothing kernel and a set of latent process.
%Another line of high dimensional GP is based on convolution method between a smoothing kernel and a set of latent functions~\citep{higdon2002space,boyle2005dependent,teh2005semiparametric, bonilla2008multi}.
Despite their elegance, these methods are normally computationally costly. 
They have $\Ocal(N^3d^3)$ time complexity and hence are inappropriate for our application where the dimension is extremely large (\eg 1 million) while the samples are limited.
